Algorithmic Persuasion Through Simulation

We study a Bayesian persuasion game where a sender wants to persuade a receiver to take a binary action, such as purchasing a product. The sender is informed about the (real-valued) state of the world, such as the quality of the product, but only has limited information about the receiver's beliefs and utilities. Motivated by customer surveys, user studies, and recent advances in AI, we allow the sender to learn more about the receiver by querying an oracle that simulates the receiver's behavior. After a fixed number of queries, the sender commits to a messaging policy and the receiver takes the action that maximizes her expected utility given the message she receives. We characterize the sender's optimal messaging policy given any distribution over receiver types. We then design a polynomial-time querying algorithm that optimizes the sender's expected utility in this game. We also consider approximate oracles, more general query structures, and costly queries.

==> paper/main_body/acks.tex <==
\section*{Acknowledgements}
%
The authors would like to thank Yiding Feng for pointing out an error in a previous version of the proof of~\Cref{prop:opt-binary}.
%
The authors would like to thank James Best, the participants of the DIMACS Workshop on Foundation Models, Large Language Models, and Game Theory, and the participants of the SLMath workshop on Algorithms, Approximation, and Learning in Market and Mechanism Design for helpful comments and discussions.

==> paper/main_body/adaptive_qp.tex <==
\section{Adaptive Querying Policies}\label{sec:adaptive}
%
\begin{algorithm}[t]
\caption{Computing the Optimal Adaptive Querying Policy: $K$ Queries}\label{alg:dp}
\begin{algorithmic}
\Require Query budget $K \in \mathbb{N}$\\
%
\begin{itemize}
    \item Set 
    %
    \begin{equation*}
        V[\cT', 0] := \mathbb{E}_{\tau \sim \cP(\cT')} \mathbb{E}_{\omega \sim \vp_{\tau}} \mathbb{E}_{m \sim \sigma^*_{\cP(\cT')}(\omega)} u_S(\omega, m)
    \end{equation*}
    %
    %$V[\cT', 0] := \mathbb{E}_{\tau \sim \cP(\cT')} \mathbb{E}_{\omega \sim \vp_{\tau}} \mathbb{E}_{m \sim \sigma^*_{\cP(\cT')}(\omega)} u_S(\omega, m)$ 
    %
    for all feasible receiver subsets $\cT' \in \cF_{\cT}$, where $\sigma^*_{\cP(\cT')}$ is the optimal messaging policy for receiver subset $\cT'$, as defined in~\Cref{thm:opt-sp}. 
    %
    \item For every $1 \leq k \leq K$ and all $\cT' \in \cF_{\cT}$, compute 
    %
    \begin{equation*}
        V[\cT', k] := \max_{q \in \cQ} V[\cT', k, q],
    \end{equation*}
    %
    %$V[\cT', k] := \max_{q \in \cQ} V[\cT', k, q]$, 
    %
    where 
    %
    \begin{equation*}
        V[\cT', k, q] := \sum_{i=1}^{n_q} V[\cT' \bigcap s_{q,i}, k-1] \cdot \mathbb{P}_{\cP}(\tau^* \in \cT' \bigcap s_{q,i} | \tau^* \in \cT').
    \end{equation*}
    %
    %$V[\cT', k, q] := \sum_{i=1}^{n_q} V[\cT' \bigcap s_{q,i}, k-1] \cdot \mathbb{P}_{\cP}(\tau^* \in \cT' \bigcap s_{q,i} | \tau^* \in \cT')$.
    %
    \item The optimal adaptive querying policy then makes query 
    %
    \begin{equation*}
        \pi^*(\cT' | k) = \arg\max_{q \in \cQ} V[\cT', k, q]
    \end{equation*}
    %
    %$\pi^*(\cT' | k) = \arg\max_{q \in \cQ} V[\cT', k, q]$ 
    %
    when in receiver subset $\cT'$ with $k$ queries left.
\end{itemize}
%
\end{algorithmic}
\end{algorithm}
%
We now shift our focus to computing the optimal querying policy when the sender can adaptively select $K$ queries from a set of allowable partition queries $\cQ$ (as defined in~\Cref{def:query}). 
%
Specifically, we are interested in adaptively selecting $K$ queries in such a way that maximizes the sender's utility in expectation when she messages according to the optimal messaging policy for the realized belief subset.\looseness-1 
%
\begin{definition}[Feasible Belief Subset]\label{def:feasible}
    %
    For a fixed query budget $K$, we say that a subset of receiver beliefs $\{\vp_{\tau} | \tau \in \cT'\}$ for $\cT' \subseteq \cT$ is \emph{feasible} if there exists some $\tau \in \cT$ and $\cQ' \subseteq \cQ$ with $|\cQ'| \leq K$ such that $\{\vp_{\tau} | \tau \in \cT'\} = \bigcap_{q \in \cQ'} s_{q, i(\tau)}$. 
    %
    We call $\cT'$ the corresponding feasible receiver subset. 
    %
    We denote the set of feasible belief subsets (resp. receiver subsets) by $\cF$ (resp. $\cF_{\cT}$) and the number of feasible subsets by $F := |\cF| \leq 2^K$.\looseness-1 
\end{definition}
%
%  
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/policy_tree.png}
    \caption{Game tree between sender and nature for a setting with two queries $q_1$ and $q_2$. Each query results in two feasible subsets, with query $q_1$ (resp. $q_2$) resulting in subsets $s_{q_1, 1}$ and $s_{q_1, 2}$ (resp. $s_{q_2, 1}$ and $s_{q_2, 2}$). 
    %
    Sender actions (black circles) are queries to the oracle, and nature actions (white squares) are (refined) subsets of receiver beliefs. No matter what subset of receiver types $\cT' \in \cF_{\cT}$ is reached, the probability of reaching $\cT'$ is exactly equal to $\cP(\cT')$ by construction.}
    \label{fig:game-tree}
\end{figure}
%
%
An adaptive querying policy needs to specify a query to make for each of the $F$ feasible belief subsets.
%
%Observe that the sender's optimal query for a particular receiver subset $\cT'$ may depend on any future queries which are made, but it does not depend on the queries which led to the sender being in subset $\cT'$. 
%
Observe that the sender's optimal querying policy starting from receiver subset $\cT'$ is independent of any queries used previously to refine the subset, but may need to anticipate future queries. 
%
For example, consider an instance of Binary BP with four possible receiver types and $K=2$ simulation queries. 
%
In this scenario, it will always be optimal to use the first query to separate the smallest two receiver beliefs from the largest two beliefs, \emph{regardless of the immediate utility gain from doing so or any other parameters of the problem instance}, since this allows the second query to fully separate all receiver beliefs. 
%
Any other initial query is always strictly suboptimal. %if there is positive benefit from separating each pair of beliefs.
%

Motivated by the necessity of anticipating future queries, we show that the sender's optimal querying policy may be computed via backward induction on an appropriately-constructed extensive-form game tree. 
%
We start by considering the expected utility associated with the optimal messaging policy for each belief subset whenever the sender has no queries remaining. 
%
Using these expected utilities as a building block, we can compute the sender's optimal querying policy when she has only one query. 
%
We then use our solution for one query to construct the optimal querying policy whenever the sender has two queries, and we continue iterating until we have the optimal adaptive querying policy for $K$ queries. 
%
This process is illustrated in~\Cref{fig:game-tree} and formally described in~\Cref{alg:dp}. 
%
\begin{restatable}{theorem}{thmdp}\label{thm:DP}
    \Cref{alg:dp} computes the sender's optimal adaptive querying policy for $K$ partition queries in $\mathcal{O}(FKQT)$ time.
    %
    In Binary BP with simulation queries, the runtime is $\mathcal{O}(T^4K)$.
\end{restatable}
%
Note that computing the optimal adaptive policy via brute-force search requires considering $\mathcal{O}(Q^F)$ policies and since $F \leq 2^K$,~\Cref{alg:dp} allows us to go from doubly-exponential-in-$K$ to exponential-in-$K$ time in the worst case. %(as $Q$ can be as large as $T^K$ in the worst case). 
%
In order to separate the time it takes to compute the optimal \emph{querying} policy from any time required to compute the sender's \emph{messaging} policy, we assume that the optimal messaging policies for each feasible belief subset are known to the sender before~\Cref{alg:dp} is run. 
%
Alternatively, one could view the computation of the optimal messaging policies as part of~\Cref{alg:dp}, in which case the runtime would contain an additional additive factor proportional to the time it takes to compute the optimal messaging policy under uncertainty (see~\Cref{thm:opt-sp}). 
%


==> paper/main_body/committing_to_query.tex <==
\section{Extension: Committing to Query}\label{sec:committing}
%
\begin{figure}[t]
    \centering
    \noindent \fbox{\parbox{0.9\textwidth}{
    \vspace{0.1cm}
    \textbf{Protocol: Bayesian Persuasion with Commitment to Query}
    
    \vspace{-0.3cm}
    %\noindent\rule{15.9cm}{0.4pt}
    %\noindent\rule{14.9cm}{0.4pt}
    \noindent\rule{12.5cm}{0.4pt}\vspace{1mm}
    %\vspace{-0.7cm}
    \begin{enumerate}
        %\setcounter{enumi}{-1}
        \item Sender commits to querying policy $\pi : \Omega \rightarrow \cQ$ and messaging policy $\sigma : \Omega \times \cS \rightarrow \cM$.
        %
        \item Sender observes state $\omega \sim \vp_{\tau^*}$, where $\tau^* \sim \cP$ is the true receiver type.
        %
        \item Sender makes query $q = \pi(\omega)$ and observes receiver subset $s$.
        %
        \item Sender sends message $m \sim \sigma(\omega, s)$, receiver forms posterior 
        $\rbr{\vp_{\tau^*} \mid m, \sigma}$.
        %
        \item Receiver takes action $\arg\max_{a \in \cA} \mathbb{E}_{\omega \sim \vp_{\tau^*}}\sbr{u_R(\omega, a) \mid  m, \sigma, \pi}$.
    \end{enumerate}
    }}
    \caption{Description of the Bayesian Persuasion game between a sender and receiver, when the sender can commit to a querying policy.}
    \label{fig:summary-commit}
\end{figure}
%
In line with the classic BP setup, we have so far assumed that the sender has the ability to commit to a messaging policy, but must make all of her oracle queries before seeing the state. 
%
In this section, we explore the effects of \emph{further} commitment power on the sender's side; namely, the power to commit to a querying policy. 
%
We focus on the simplified setting in which the sender can make one costless query ($K=1$), for which there is no difference between adaptive and non-adaptive querying policies. 
%
Unlike in the previous setting without this extra commitment power, the sender's querying policy can now depend on the realized state, and her messaging policy can depend on both the state \emph{and} the outcome of the query.  
%
\begin{definition}[State-Informed Querying Policy]
    A querying policy $\pi : \Omega \rightarrow \cQ$ is \emph{state-informed} if the query made depends on the state realization.
\end{definition}
%
Similarly, a messaging policy is \emph{subset-informed} if the realized message depends on both the realized state and the outcome of the query. 
%
\begin{definition}[Subset-Informed Messaging Policy]
    A messaging policy $\sigma : \Omega \times \cS \rightarrow \cM$ is \emph{subset-informed} if the message sent depends on the realized belief subset. 
\end{definition}
%
Note that a subset-informed messaging policy is different than a messaging policy which operates on a refined subset of receiver beliefs. 
%
In particular, a subset-informed messaging policy takes a subset of beliefs as input (in addition to the state) and produces a message.
%
In contrast, our previous definition of a messaging policy (\Cref{def:messaging}) does not take any information about receiver belief subsets as input. 
%

See~\Cref{fig:summary-commit} for a summary of the updated interaction protocol under additional commitment.
%
Note that the ability to commit to a state-informed querying policy will never hurt the sender, since the sender has the option of choosing a state-independent querying policy.
%
On the other hand, the sender can sometimes benefit substantially from this additional commitment power, as the following example illustrates.\looseness-1
%The following example illustrates how the sender can benefit from this additional commitment power.\looseness-1 
%
\begin{example}\label{ex:query-after} 
%
Consider the following natural extension of Binary BP with simulation queries to three states and actions: 
%
Let $\Omega = \{-1, 0, 1\}$, $\cA = \{-1, 0, 1\}$, $u_S(\omega, a) = a$, and $u_R(\omega, a) = \mathbbm{1}\{a = \omega\}$. 
%
Let $\cQ$ be the set of simulation queries and consider the set of receivers $\cT = \{\tau_1, \tau_2, \tau_3\}$ with respective beliefs 
%
\begin{equation*}
\begin{aligned}
    \vp_1 &= [0.75, 0.25, 0],\\
    %
    \vp_2 &= [0.75+\delta, 0, 0.25-\delta], \text{ and}\\
    %
    \vp_3 &= [0, 0.75+\epsilon, 0.25-\epsilon]
\end{aligned}
\end{equation*}
%$\vp_1 = [0.75, 0.25, 0]$, $\vp_2 = [0.75+\delta, 0, 0.25-\delta]$, $\vp_3 = [0, 0.75+\epsilon, 0.25-\epsilon]$ 
%
for some $\epsilon, \delta > 0$. 
%
\end{example}
%
Observe that in the setting of~\Cref{ex:query-after}, after seeing the state realization the sender will always be able to rule out one of the receiver beliefs (since they all put zero probability mass on a different state), and thus she can use her query to distinguish between the remaining two beliefs. 
%
If the sender commits to messaging according to the optimal messaging policy for the realized belief, this procedure is BIC since the sender will always send a message to a receiver of type $i$ using messaging policy $\sigma_i^*$ for every possible state realization. 
%
Note that if the sender queried the oracle \emph{before} seeing the state, she would not always be able to distinguish between all three beliefs. 
%
%
See~\Cref{fig:state_first} for a visualization of this setting. 
%

Equipped with this intuition as to how committing to query can help the sender, we return to Binary BP with simulation queries. 
%
\begin{definition}\label{def:implement}
    We say that a subset-informed messaging policy $\sigma$ \emph{implements} a messaging policy $\sigma_i$ for receiver type $\tau_i$ if 
    %
    \begin{equation*}
        \sigma_i(a | \omega) = \sum_{m \in \cM : m[i] = a} \sigma(m | \omega)
    \end{equation*}
    %
    %$\sigma_i(a | \omega) = \sum_{m \in \cM : m[i] = a} \sigma(m | \omega)$ 
    %
    for all $\omega \in \Omega$, $a \in \cA$.
\end{definition}
%
In other words, a subset-informed messaging policy $\sigma$ can implement a (subset-uninformed) messaging policy $\sigma_i$ from receiver type $i$'s point of view if they cannot distinguish between the two after aggregating all of the messages which recommend them to take action $a$, for every $a \in \cA$. 
%
\begin{restatable}{theorem}{threepolicy}\label{thm:threepolicy}
    Given any three messaging policies $\sigma_1$, $\sigma_2$, $\sigma_3$ where $\sigma_1$ (resp. $\sigma_2$, $\sigma_3$) is an arbitrary messaging policy which is Bayesian incentive-compatible for agents of type $\tau_1$ (resp. $\tau_2$, $\tau_3$), there exists a BIC state-informed querying policy and subset-informed messaging policy which can implement $\sigma_1$, $\sigma_2$, and $\sigma_3$ simultaneously (according to~\Cref{def:implement}).
\end{restatable}
%
The result follows from writing down the problem of designing a BIC querying and messaging policy in this setting as a linear constraint satisfaction problem (CSP), and showing that this CSP still has a feasible solution whenever additional constraints are added to ensure that $\sigma_1$, $\sigma_2$, and $\sigma_3$ are implemented. 
%
Note that it is generally only possible to implement \emph{two} messaging policies for different receiver beliefs when querying \emph{before} seeing the state.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/state_first.png}
    \caption{Visualization of~\Cref{ex:query-after}. Left: Seeing the state helps the sender because it allows them to eliminate one receiver type before querying the oracle. Right: The procedure described in~\Cref{ex:query-after} is incentive-compatible for the receiver because the messaging policy faced by any individual receiver type will be the same (namely, the sender's optimal messaging policy for that type), regardless of the state realization.}
    \label{fig:state_first}
\end{figure}

==> paper/main_body/conc-old.tex <==
\section{Conclusion and Future Work}\label{sec:conc}
%

We initiate the study of information design with an oracle, motivated by recent advances in large language models and generative AI, as well as more traditional settings such as experimentation on a small number of users. We study a setting in which the sender in a Bayesian persuasion problem can interact with an oracle for $K$ rounds before trying to persuade the receiver. After showing how the sender can reason about messaging under uncertainty and can benefit from this additional query access, we show how to derive the sender's optimal adaptive querying policy via dynamic programming. 

Next we show that while in the general setting, computing the sender's optimal non-adaptive querying policy is an NP-Complete problem, it can be solved for efficiently via dynamic programming in Binary BP with simulation queries. 
%
Motivated by this observation, we study the sender's expected utility as a function of the queries they make. 
%
We find that the sender's expected utility exhibits decreasing marginal returns as a function of additional queries in Binary BP. 
%
In contrast, this property does not hold in the general setting, which rules out the possibility of achieving good approximation algorithms using the greedy heuristic. 
%
Finally, we explore the effects of additional commitment power on the sender's querying policy and find that this additional commitment can significantly benefit the sender. 
%

There are several exciting directions for future research. 
%
While we focus on Bayesian Persuasion for its simplicity and ubiquity, it would be interesting to study the benefits of oracle access in other information design settings, such as cheap talk \cite{crawford1982strategic} or verifiable disclosure \cite{grossman1980disclosure}. 
%
Throughout this work, we assume that the sender has access to an oracle which is able to \emph{perfectly} simulate the receiver. 
%
However in reality the oracle may make mistakes. 
%
%An LLM may not be able to perfectly replicate the behavior of the person it is being used to simulate. 
%
%Agents used for pure exploration may not be representative of the larger population. 
%
An interesting direction is to analyze the performance of our methods whenever the oracle is allowed to be imprecise, and if necessary, modify our algorithms to be robust to such misspecification. 
%
Finally while the focus of our work is on settings in which the receiver's utilities are known and the sender is uncertain about the receiver's beliefs, it would be natural to ask how oracle access could help the sender achieve higher utility whenever the receiver's utility function is unknown. 

==> paper/main_body/intro-v1.tex <==
\section{Introduction}
%
\emph{Bayesian Persuasion}~\cite{kamenica2011bayesian, kamenica2019bayesian} is a game of asymmetric information between two players: an informed \emph{sender}, who observes the \emph{state} of the world, and an uninformed \emph{receiver}, who does not see the state but takes an \emph{action}. 
%
The payoffs of both players depend on both the world's state and the receiver's action. 
%
The game proceeds as follows: 
%
The sender commits to a \emph{signaling policy}, i.e. a mechanism for revealing information to the receiver about the state of the world, before the state is realized. 
%
Once the state is realized, the sender sends a signal (or \emph{message}) to the receiver according to their signaling policy. 
%
Upon receiving the signal, the receiver updates their belief about the state of the world, and takes an action.
%
One motivating example of the Bayesian Persuasion framework is the interaction between a \emph{seller} of a product (the sender) and a potential \emph{buyer} (the receiver), where the state of the world is the quality of the product (e.g. high/low quality). 
%
The seller would always like to sell the product to the buyer, but the buyer only wants to purchase the product if it is of high quality.
%\footnote{The seller's ability to commit may arise from, e.g. legal regulations or the seller's desire to protect their reputation.}

%In many persuasion settings, the sender can only compute the payoff-maximizing signaling policy whenever they have \emph{full information} about the receiver (e.g. knowledge of the receiver's \emph{belief} about the true state of the world). 
%
The sender's payoff-maximizing signaling policy often depends on information about the receiver which may not be known to the sender; for example, the receiver's \emph{belief} about the true state of the world. 
%
This observation has motivated a line of work on \emph{robust} Bayesian Persuasion (e.g. \cite{dworczak2022preparing, parakhonyak2022persuasion, hu2021robust}), which broadly aims to determine the sender's optimal signaling policy when almost \emph{no information} is known about the receiver.
%
While robust signaling policies are applicable in a wider range of settings when compared to methods which require \emph{full information} about the receiver, they are not without their drawbacks. 
%
Perhaps unsurprisingly, signaling policies which use information about the receiver are more persuasive and are often simpler when compared to their robust counterparts. 
%
This raises the question: 
\vspace{-3mm}

{\centerline \em \textit{How can the sender design simple, persuasive signaling policies when they initially have minimal information about the receiver?}}
\vspace{2mm}

%
One useful observation is that in many settings of interest, the sender is not at either end of the informational spectrum, but instead may \emph{acquire} additional information about the receiver through external sources. 
%
For instance, the sender may be able to learn about the receiver's beliefs through one of the following processes:
%
\begin{enumerate}
    \item \textbf{Receiver simulation using Generative AI and machine learning.} 
    %
    Given sufficient data about the receiver, the sender may be able to predict the receiver's behavior under different settings using machine learning models. 
    %
    There has been recent interest in using large language models (LLMs) as \emph{simulated economic agents} which can be endowed with preferences or beliefs and used to obtain insights about how humans may behave in real-world strategic scenarios (e.g.~\cite{horton2023large, fish2023generative}). 
    %
    Suppose the sender uses an LLM, fine-tuned with relevant data about the receiver, to try out different methods of information disclosure before attempting to persuade the receiver. 
    %
    As another example, suppose the seller is an online marketplace who wants to bring a new product to market and the buyer is a marketplace user. 
    %
    While the seller may initially be unsure about how the new product will be received, they may be able to use the user's purchase history on the platform to predict something about how the user would respond to a sales pitch for the new product. 
    %
    Finally if the receiver is itself an AI agent, it may be possible to simulate the receiver directly. 
    %
    \item \textbf{Simulation as a metaphor for exploration.} The sender may be able to learn about the behavior of the receiver through their interactions with other receivers in the past. 
    %
    For example, a startup may test out their sales pitch on smaller venture capital firms before trying to persuade a larger firm to fund their business. 
    %
    A company may run a focus group on a small set of customers before bringing a new product to market.  
    %
    More generally, it may be possible for the sender to conduct market research about the receiver before trying to persuade them. 
    %
\end{enumerate}
%
Motivated by such settings, we consider an idealized model in which the sender in a Bayesian Persuasion game has access to an \emph{oracle} with information about the receiver. 
%
The sender can \emph{query} the oracle, and each query reveals a piece of information about the receiver, possibly at some \emph{cost} to the sender. 
%
Given a set of allowable queries, we are interested in (1) analyzing how querying the oracle can help the sender design more persuasive signaling policies and (2) determining the sender's optimal \emph{querying policy} when given a \emph{budget} on the number of queries allowed.\looseness-1 

\iffalse
So what type of information can the sender acquire? 
%
Information about receiver beliefs is almost never \emph{directly} observable, but in many settings the sender can obtain \emph{indirect} information about the receiver's beliefs before or during the interaction.\footnote{While the receiver could (in principle) reveal their beliefs to the sender, it may not be in their best interest to report their beliefs truthfully. 
%
Furthermore, it is unclear whether the receiver would even be able to accurately express their beliefs in some settings.}  
%
In the context of the sales example, the seller may be able to infer something about the buyer's beliefs about the quality of the product by observing whether or not they purchase the product.\looseness-1

Depending on the setting of interest, the sender may be able to \emph{simulate} revealed preference feedback even before they send a signal. 
%
Consider the following three motivating examples:
%
\begin{enumerate}
    %
    \item Due recent to advances in generative AI, there has been interest in using large language models (LLMs) as \emph{simulated economic agents} (e.g.~\cite{horton2023large, fish2023generative}). 
    %
    Suppose the sender uses an LLM, possibly fine-tuned with relevant data about the receiver, to try out different methods of information disclosure before attempting to persuade the receiver. 
    %
    \item Suppose the seller is a large online marketplace and the buyer is a marketplace user. 
    %
    If the seller has a large amount of historical data from different buyers who have visited the platform (through e.g. their purchase and search histories), as well as data about their interactions with the platform (e.g. whether or not they bought an item), the seller may be able to train a machine learning model to accurately predict how a particular user would respond when given certain information about the product they are interested in.
    %
    \item Consider a business-to-business commerce setting in which one company would like to sell a product to another company, and both companies are initially unsure about whether or not purchasing the product will end up benefiting the potential buyer. 
    %
    A natural strategy for the selling company is to hire a consulting agency to conduct market research. 
    %
    By the end of their research, the consulting firm should be able to answer certain questions the seller may have about the buyer, which may help the seller be more persuasive during their sales pitch.
    %
\end{enumerate}
\fi 

\iffalse
\khcomment{Outline of Introduction
\begin{itemize}
    %\item Motivate/ explain Bayesian Persuasion at a high level
    %
    %\item Introduce running buyer/seller example
    %
    %\item Motivate/mention robust persuasion literature: the assumption of a \emph{known} receiver prior is unrealistic! However, this lack of assumptions about what is known about the receiver often leads to signaling policies which are either overly complicated or not very persuasive (oftentimes both). 
    %
    %\item Punchline: In many settings, the sender is at neither of these two extremes. In reality, they may have some sort of imperfect information about the receiver, or they may be able to \emph{acquire} it through some process (e.g. by running an experiment, conducting a field trial, etc.). 
    %
    %\item But what type of access to receiver information is reasonable? While the sender would like to have \emph{direct} access to information about the receiver's prior, such information is not observable to them. While the receiver could (in principle) reveal information about their prior to the sender, in most settings it would not be in their best interest to do so. Moreover, it is unclear whether a receiver would even be able to express their prior in some settings.
    %
    %\item On the other hand, when interacting with a population of receivers, the sender does get to observe their \emph{revealed preferences}, i.e. given a signaling policy and message realization, the sender can observe a receiver's best response. 
    %
    %\item For example, consider an online marketplace (the sender) interested in selling to users of the platform. The sender has a large amount of historical data of the form (receiver context, signaling policy, message, receiver action), which they can use to train a machine learning model to predict the response of the receiver to a (signaling policy, message) pair
    %
    %\item Another example is business-to-business transactions. One company (the seller) is trying to sell a product to another company (the buyer), and \emph{a priori} both are unsure about whether or not the product will benefit the (potential) buyer. The seller decides to hire a consulting agency to conduct research about the buyer. By the end of their research, the consulting firm will be able to answer certain questions that the seller may have about the buyer. The answers to these questions may help the seller be more persuasive in their sales pitch
    %
    \item Motivated by such settings, we consider a sender who has \emph{simulator} access to the receiver. In other words, the sender can give an oracle a (signaling policy, message) pair, and can observe the response of the receiver, possibly at some \emph{cost}
    %
\end{itemize}
}
\fi 
%
\subsection{Overview of Our Results}
%
We discuss related work in~\Cref{sec:related}, including connections to online learning for Bayesian Persuasion, learning in Stackelberg games, and the simulation of economic agents using LLMs. 
%
In~\Cref{sec:setting}, we overview our setting and provide background on Bayesian Persuasion. 
%
In~\Cref{sec:unknown_prior}, we characterize the form of the sender's optimal signaling policy whenever the sender is uncertain about the receiver's beliefs. 
%
We explain how a natural type of oracle access which we call \emph{simulator access} can help the sender achieve higher expected utility in~\Cref{sec:helps}. 
%
In particular, borrowing language from the field of convex optimization, we show that making a simulation query is equivalent to specifying a subset of ``receiver belief space'' to which the sender has \emph{separation oracle} access. 
%
If the receiver's true beliefs fall within the specified subset, the separation oracle says so. 
%
Otherwise, it returns a separating hyperplane in belief space. 
%
Using this characterization, we show how it is possible to use simulation queries to decrease the sender's uncertainty about the receiver's beliefs, which leads to higher sender utility. 
%
In~\Cref{sec:adaptive} we shift our focus to computing \emph{adaptive} querying policies, where the sender's $i$-th query to the oracle can depend on the outcomes of all previous $i-1$ queries. 
%
We show that the space of adaptive querying policies can be characterized by an extensive-form game between the sender and nature, and that the optimal adaptive querying policy may be solved for via backward induction on the game tree. 
%
We consider \emph{non-adaptive} querying policies (i.e. querying policies which must make all queries \emph{up front}) in~\Cref{sec:non-adaptive}. 
%
While we show that the general problem of computing the sender's optimal non-adaptive querying policy is NP-Complete via a reduction from set cover, the problem may be solved efficiently when the sender is restricted to making simulation queries in a canonical setting with binary states and actions. 
%
Motivated by these results, we study the effects of querying on the sender's expected utility in the non-adaptive setting. 
%
In~\Cref{sec:properties} we show that the sender's expected utility is a submodular function of the queries made by the sender when there are binary states and actions. 
%
This implies that under this binary setting, there are diminishing returns to additional queries. 
%
In contrast, we show that this property does \emph{not} hold in the general setting. 
%
Using this result, we show that the \emph{greedy} policy, a popular heuristic often used to obtain approximately optimal solutions, is \emph{not} approximately optimal when learning to persuade from oracle queries. 
%
All of our positive results for both adaptive and non-adaptive querying policies extend to the setting where the sender incurs a \emph{cost} for making a query. 
%
In~\Cref{sec:committing}, we explore the setting in which the sender can \emph{commit} to a querying policy (in addition to a signaling policy). 
%
This additional commitment power never hurts the sender, and we show that it can sometimes help them significantly. 
%
Finally, we conclude and highlight directions for future research in~\Cref{sec:conc}.

==> paper/main_body/intro-v2.tex <==
\section{Introduction}\label{sec:intro}
%
Information design\footnote{See \citep{BergemannMorris-survey19} for a survey of this research area.} is a canonical branch of theoretical economics which analyzes how provision of information influences strategic behavior.
%
A typical framing involves a game with uncertain payoffs and an information designer who can commit to a particular information structure for the participants of this game.
%
The designer chooses among feasible information structures so as to maximize her utility.
%
While more idealized formulations assume that participant beliefs and preferences are fully known to the designer, in reality they often are not.\looseness-1

We initiate the study of information design with an \emph{agent-informed oracle}: an oracle endowed with information about the participant and available to the information designer.
%
%Specifically, we posit that the principal has access to an oracle endowed with information about the agents.
%
The designer can query this oracle at a cost to supplement its incomplete knowledge about the participants. 
%
The query structure of the oracle can vary from application to application, but generically it enables the designer to refine her beliefs about the participant's beliefs.
%
A salient case is a simulation oracle: an oracle that can simulate participants' strategic behavior in the game being studied, inducing a certain structure on refinements of the participant belief space.
%
Our high-level goal is to explore how access to this additional source of information can help the principal optimize the information structure.\looseness-1

We focus on Bayesian Persuasion (BP)~\cite{kamenica2011bayesian}, a paradigmatic setting in information design.
%
BP is a game of asymmetric information between two players: an informed \emph{sender} (corresponding to the designer in information design) and an uninformed \emph{receiver} (corresponding to an agent in information design).
%
The sender observes a payoff-relevant \emph{state} of the world and sends a \emph{message} to the receiver, who then chooses an \emph{action} which yields payoffs for both players.
%
The sender commits to a messaging policy before the state is revealed, and the receiver takes an action based on the realized message. %\footnote{The sender is the information designer, with the messaging policy defining the receiver's information structure.}
%
We extend this game to allow the sender to query a receiver-informed oracle
%that can provide additional information about the receiver
before she commits to a messaging policy.\looseness-1

\xhdr{Motivation.}
Agent-informed oracles are motivated by recent advances in Generative AI, particularly Large Language Models (LLMs), e.g., \cite{openai2023gpt, anil2023palm, touvron2023llama}.
%
LLMs exhibit an emergent capability to simulate strategic behavior of economic agents. 
%It has been shown that LLMs can simulate the strategic behavior of humans in economic settings.
% LLMs can simulate traditional (human-driven) experiments in behavioral economics~\cite{horton2023large}.
%
Notably, LLMs have been shown to make consumer choices that track with those of humans. 
%
They exhibit downward-sloping demand curves,
diminishing marginal utility of wealth, and state dependence, and further match the stated willingness-to-pay of consumers in a recent market survey \citep{brand2023using}. 
%
They even exhibit (sometimes non-strategic) behaviors consistent with particular demographics given appropriate framing, such as libertarians in the context of pricing \citep{horton2023large} or women in the context of ultimatum games \citep{aher2023using}.
%
Recent work also shows they can infer demographics and even user personality traits from online telemetry data such as Facebook status updates \citep{peters2023large}. 
%
Based on these experiments, and the common belief that the capabilities of LLMs will continue to improve, we argue they will be increasingly used as agent-informed oracles in information design settings.
%

An agent-informed oracle can be implemented with access to more traditional AI  as well.
%
%One could implement it via a general-purpose LLM such as GPT-4, with appropriate prompt-engineering (like in \cite{horton2023large, brand2023using}).
%
One could train a specialized machine learning model using domain-specific data, and use this model to predict strategic behavior in a particular domain.
%
Moreover, strategic parties are increasingly implemented via AI agents, \eg in online markets, ad auctions, and gaming, in which case it may be possible to simulate them directly through access to (or knowledge of) the AI agent.
%
In each of these cases, the sender must incur some cost to query the oracle.%
\footnote{For example, query costs for LLMs can be substantial, in terms of money and/or delay. In fact, the latest LLMs can be very expensive, as of this writing, if a large volume of queries is needed \cite{JGPT}.}
%notoriously high \cite{JGPT}.

An agent-informed oracle can also be a metaphor for market research that the sender performs before interacting with the receiver.
%
For example,  a startup may test out its funding pitch on smaller venture capital firms before trying to persuade a larger firm to fund their business.
%
A company may run a customer survey before bringing a new product or service to market, or experiment on a fraction of users in online services \citep[\eg][]{KohaviLSH09,KohaviAB-2015}.
%
Again, the ``queries'' in these settings are expensive; a startup may have a limited number of venture capital firms that it can pitch to, and a company may be limited in the number of customers/users it can survey without disrupting overall sales.\looseness-1

As a specific example of BP, consider the interaction between a seller (the sender) of a product with a fixed price and a potential buyer (the receiver).
%
Here, the state of the world is the quality of the product (\eg high/low quality) and the message corresponds to the sales pitch presented to the buyer.
%
The seller would always like to sell, but the buyer only wants to buy if the product is of sufficiently high quality.
%
A buyer-informed oracle may help the seller optimize her sales pitch. 
%
In BP, the seller must commit to this sales pitch before observing the product quality; this ability to commit may arise from, e.g. legal regulations or the seller's desire to protect her reputation.  
%
This is a rather general scenario: the ``product" may refer to a physical good as well as any service, opportunity, or experience; the ``quality" may be absolute and/or buyer-specific; the ``sales pitch" encompasses any information presented to the buyer.

A buyer-informed oracle is particularly salient in the context of an online platform that interacts with many potential buyers.
%
Economies of scale may enable a sophisticated automatic workflow with an AI-based oracle, particularly algorithms that choose how to query the oracle and how to use its output to shape buyer-facing communication.
%
This communication can potentially be customized to a particular product and a particular customer.
%
The oracle itself may be either general-purpose or domain-specific, and provided by either a third party or developed within the platform.

\xhdr{Our model.}
%
We study Bayesian Persuasion (BP) with a receiver-informed oracle.
%
A problem instance consists of three parts: a BP instance, an oracle, and a cost model.

We introduce a version of BP in which the sender is endowed with partial knowledge of receiver's belief, as expressed by a second-order prior, and full knowledge of the utility structure. 
%
The state is drawn from the receiver's belief, which is in turn drawn from the sender's second-order prior.
%
This is a natural midpoint between two extremes studied in prior work.
%
The traditional formulation of BP assumes a known utility structure and a common prior on the state, so the receiver is fully known.
%
In contrast, in \emph{robust} BP \citep[\eg][]{dworczak2022preparing, parakhonyak2022persuasion, hu2021robust} the receiver is almost fully \emph{not} known.

The sender can query the oracle to gain additional information about the receiver's belief.%
\footnote{
Of course, oracle queries may also reveal information about the state, since the state is drawn from the receiver's belief.  However, crucially, the oracle cannot reveal anything about the state that the receiver does not already know.  The power to commit to a messaging policy before the state is revealed is therefore still valuable to the sender.
%The oracle may also reveal some information about the state (because it is drawn from the receiver's belief), but since the oracle does not reveal anything about the state that the receiver does not already know, the commitment power in BP is still valuable to the sender.
%The oracle does not reveal anything that the receiver does not already know. In particular, while the oracle may reveal some information about the state (because it is drawn from the receiver's belief), this information would already be known to the receiver (because the receiver knows her own belief).
}
%
A generic oracle takes some input (a query) and deterministically maps it to some output, where the output is determined by the input and the true (receiver) belief/prior.
%
The set of all possible inputs and the mapping are known to the sender.
%
Equivalently, the oracle inputs a partition of the \emph{belief space} (the set of feasible beliefs of the receiver) and returns the subset of this partition which contains the receiver's true belief.
%
We refer to this generic class of oracles as \emph{partition oracles}, and characterize it by the set of all feasible partitions of belief space.
%
A paradigmatic special case is a \emph{simulation oracle}, which simulates the receiver's response in the same BP instance.
%
Such an oracle inputs a messaging policy and a particular message realization, and outputs the action that would have been chosen by the receiver with true belief upon seeing this policy and this message. This special case is strongly motivated by the applications discussed previously.
%e.g., experimentation on a subset of users.
% AS: Keegan, this commented-out clause seems to deemphasize LLM motivation, which I think is unwise here.

Before the BP game starts, the sender (i) queries the oracle according to some \emph{querying policy} and (ii) computes a messaging policy using the information gained from the oracle.
%
The sender strives to optimize her Bayesian-expected utility, given the cost model for the oracle.
%
The main cost model we consider is a \emph{query budget}: a fixed number of queries that may be posed to the oracle.
%
Our results also extend to per-query costs that are subtracted from sender's utility; these costs are known to the sender \emph{a priori}, and may be different for different queries.

\xhdr{Our results.}
From an algorithmic perspective, our goal is to implement steps (i,ii) above so as to optimize the sender's Bayesian-expected utility.
%
Our technical analysis is mainly concerned with the problem of computing an optimal querying policy for step (i), assuming that an optimal messaging policy is chosen in step (ii). 
%
For the cases when we have an efficient algorithm for this problem, optimizing the messaging policy in step (ii) can be done efficiently without much difficulty.

We distinguish between \emph{adaptive} querying policies that can choose the next query after seeing the output of the previous one and \emph{non-adaptive} querying policies which must make all queries up front. We show that an optimal adaptive querying policy, for any given partition oracle, can be found via backward induction in time linear in the (worst-case) size of such policy. 
%
While the worst-case size of the policy can be exponential in the query budget, naive brute-force search takes doubly-exponential time to compute an optimal adaptive querying policy.


In contrast, computing an optimal non-adaptive querying policy (\ie an optimal subset of queries) is NP-Complete for partition oracles.
%
In fact, this holds even for a canonical ``binary'' case of BP when there are only 2 states and 2 actions (\emph{Binary BP}), e.g., high/low quality and buy-or-not in the buyer-seller BP example.
%
Even the greedy algorithm, a natural heuristic often used for approximation, provably fails in the general setting, although, as implied by the diminishing value of queries discussed below, it is approximately optimal in the Binary BP setting.
%
On the other hand, we provide a polynomial-time algorithm for Binary BP with a simulation oracle.
%
%We take advantage of the fact that there is a total ordering over oracle queries under this setting
We find that oracle queries are totally ordered, and we leverage this ordering to compute an optimal querying policy via dynamic programming.\looseness-1

% all dim-returns: all for non-adaptive
% positive results: Binary BP, simulation queries
% negative results: example, beyond Binary BP, partition queries

% commitment power result: example {2 states, 1 simulation query}

We also provide structural insights. First, we are interested in the diminishing returns property in terms of the number of queries the sender makes to the oracle.%
\footnote{In other words, whether the marginal utility of adding one more oracle query decreases with the query budget.}
%
We establish this property for Binary BP with a simulation oracle.
%
However, this property does not hold in general: we provide a counterexample with a specific (non-binary) BP instance and a specific partition oracle.
%
Second, we consider the effect of allowing the sender to \emph{commit} to a particular querying policy.
%
We find that this additional commitment power cannot hurt the sender, and can sometimes significantly benefit her utility.\looseness-1 
%
%For the latter result, we provide a simple example when the sender is allowed to make a single costless query.\looseness-1 

==> paper/main_body/list_of_figures.tex <==
\section{Figures}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/best-response-regions.png}
    \caption{Visualization of receiver best-response regions in $\Delta^d$ for simulation query $q = (\sigma_q, m_q)$.
    %
    On the left, the receiver follows the sender's recommendation, and we can infer that her belief $\vp_{\tau^*}$ is contained in the best-response region for $a_2$. 
    %
    On the right, the receiver does not follow the sender's recommendation, and we can instead infer that her belief is in the best-response region for $a_3$.\looseness-1}
    \label{fig:br-regions}
\end{figure}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/policy_tree.png}
    \caption{Game tree between sender and nature for a setting with two queries $q_1$ and $q_2$. Each query results in two feasible subsets, with query $q_1$ (resp. $q_2$) resulting in subsets $s_{q_1, 1}$ and $s_{q_1, 2}$ (resp. $s_{q_2, 1}$ and $s_{q_2, 2}$). 
    %
    Sender actions (black circles) are queries to the oracle, and nature actions (white squares) are (refined) subsets of receiver types. No matter what subset of receiver types $\cT' \in \cF$ is reached, the probability of reaching $\cT'$ is exactly equal to $\cP(\cT')$ by construction.}
    \label{fig:game-tree}
\end{figure}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\textwidth]{figures/bin-dp.png}
    \caption{Sender's expected utility $u(i')$ (y-axis) as a function of the cutoff receiver index $i'$ in Binary BP. Under this problem instance there are five types with beliefs $p_1 = 0.5$, $p_2 = 0.4$, $p_3 = 0.3$, $p_4 = 0.2$, and $p_5 = 0.1$ (x-axis), and second-order prior $\cP(\tau_1) = 0.2$, $\cP(\tau_2) = 0.01$, $\cP(\tau_3) = 0.39$, $\cP(\tau_4) = 0.2$, and $\cP(\tau_5) = 0.2$. 
    %
    (Recall the form of the optimal messaging policy in~\Cref{cor:opt-binary}.)
    %
    Blue: Sender's utility as a function of the cutoff index when they make no queries. 
    %
    The sender's optimal utility is given by the blue dashed line. 
    %
    Red: Sender's utility as a function of cutoff index when they make the simulation query $q$ which separates $\{\tau_1, \tau_2, \tau_3\}$ from $\{\tau_4, \tau_5\}$. 
    %
    The red dashed line denotes the sender's utility from messaging optimally after making query $q$.
    %https://www.desmos.com/calculator/hdun0wsdk3
    }
    \label{fig:bin-dp}
\end{figure}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\textwidth]{figures/fig-submod.png}
    \caption{Submodularity in Binary BP with simulation queries. 
    %
    Under this problem instance there are five types with beliefs $p_1 = 0.5$, $p_2 = 0.4$, $p_3 = 0.3$, $p_4 = 0.2$, and $p_5 = 0.1$ (x-axis), and second-order prior $\cP(\tau_1) = 0.2$, $\cP(\tau_2) = 0.01$, $\cP(\tau_3) = 0.39$, $\cP(\tau_4) = 0.2$, and $\cP(\tau_5) = 0.2$. 
    %
    (Recall the form of the optimal messaging policy in~\Cref{cor:opt-binary}.)
    %
    Blue: Sender's utility as a function of the cutoff index. 
    %
    Red: Sender's utility as a function of cutoff index when they know the true receiver belief is either $p_2$, $p_3$, or $p_4$ from previous queries. 
    %
    Blue and red crosses denote the sender's expected utility after query $q$ is made. 
    %
    The black cross denotes both a blue and red cross on top of one another. 
    %
    The blue and red dashed lines denote the sender's respective marginal gains in utility from messaging optimally after making query $q$. 
    %
    The marginal gain is always higher when the sender has more uncertainty over the receiver's true type. 
    %see desmos.com
    }
    \label{fig:submod}
\end{figure}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/bad_ex.png}
    \caption{Illustration of~\Cref{ex:greedy-bad2} in two dimensions. 
    %
    Under this setting, there are four receiver types $\tau_1$, $\tau_2$, $\tau_3$, $\tau_4$ and two queries. 
    %
    Query $q_1$ separates $\tau_1$ and $\tau_3$ from $\tau_2$ and $\tau_4$. 
    %
    Query $q_2$ separates $\tau_1$ and $\tau_2$ from $\tau_3$ and $\tau_4$. 
    %
    The sender and receiver utilities are constructed in such a way that the sender's expected utility only increases after making both $q_1$ and $q_2$.}
    \label{fig:bad-ex}
\end{figure}
%
%
\begin{figure}[!htb]
    \centering
    \noindent \fbox{\parbox{0.9\textwidth}{
    \vspace{0.1cm}
    \textbf{Protocol: Bayesian Persuasion with Commitment to Query}
    
    \vspace{-0.3cm}
    %\noindent\rule{15.9cm}{0.4pt}
    \noindent\rule{14.9cm}{0.4pt}
    %\noindent\rule{13.2cm}{0.4pt}\vspace{1mm}
    \vspace{-0.7cm}
    \begin{enumerate}
        %\setcounter{enumi}{-1}
        \item Sender commits to querying policy $\pi : \Omega \rightarrow \cQ$ and messaging policy $\sigma : \Omega \times \cS \rightarrow \cM$\vspace{-2mm}
        %
        \item Sender observes state $\omega \sim \vp_{\tau^*}$, where $\tau^* \sim \cP$.\vspace{-2mm}
        %
        \item Sender makes query $q = \pi(\omega)$ and observes information partition $s$.\vspace{-2mm}
        %
        \item Sender sends message $m \sim \sigma(\omega, s)$, receiver forms posterior $\vp_{\tau^*} | m$.\vspace{-2mm}
        %
        \item Receiver takes action $a_R := \arg\max_{a \in \cA} \mathbb{E}_{\omega \sim \vp_{\tau^*}}[u_R(\omega, a) | m]$.\vspace{-2mm}
    \end{enumerate}
    }}
    \caption{Description of the Bayesian Persuasion game between a sender and receiver, when the sender can commit to a querying policy.}
    \label{fig:summary-commit}
\end{figure}
%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/state_first.png}
    \caption{Visualization of~\Cref{ex:query-after}. Left: Seeing the state helps the sender because it allows them to eliminate one receiver type before querying the oracle. Right: The procedure described in~\Cref{ex:query-after} is incentive-compatible for the receiver because the messaging policy faced by any individual receiver type will be the same, regardless of the state realization.}
    \label{fig:state_first}
\end{figure}
%

==> paper/main_body/model-old.tex <==
\xhdr{Receiver-Informed Oracle.}
%
We are now ready to introduce the receiver-informed oracle. 
%
We consider a setting in which there are a finite set of receiver \emph{types} $\cT$ ($T := |\cT| < \infty$), where each type $\tau \in \cT$ has corresponding \emph{belief} $\vp_{\tau}$ over $\Omega$. 
%
%
We refer to the set $\{\vp_{\tau}|\tau\in\cT\}$ as the receiver \emph{belief space}. 
%
We denote the \emph{true} receiver type by $\tau^*$, and assume that $\omega \sim \vp_{\tau^*}$ (i.e. the receiver is \emph{informed} about the state in the sense that her beliefs are correct). 
%
We denote the sender's prior over receiver types (alternatively, over receiver beliefs) by $\cP(\cT)$, and assume that $\tau^* \sim \cP$. 
%
One may view $\cP(\cT)$ as a ``second-order prior'' which captures the sender's information about the receiver population in aggregate. 
%
In~\Cref{sec:uninformed} we describe how to extend our results to the setting in which the receiver is \emph{misinformed} about the state.\looseness-1

%
We consider a sender with access to an \emph{oracle} which can provide information about the receiver's belief. 
%
%In particular, we suppose that the sender can ask the oracle questions 
An oracle is characterized by the set of allowable \emph{queries} $\cQ$ with $Q := |\cQ| < \infty$, that the sender can pose. 
%The sender can pose \emph{queries} from a set $\cQ$ of allowable queries, with $Q := |\cQ| < \infty$. 
%
A particular query can be represented via a deterministic mapping from beliefs to the possible answers.  
%
To abstract away from details of the query implementation, we adopt an equivalent definition in terms of how the possible answers to the query partition the belief space.
%
\begin{definition}[Partition Oracles and Partition Queries]\label{def:query}
    %
    A partition query $q \in \cQ$ is a partition of the receiver belief space into a set of $n_q$ non-overlapping subsets $\{s_{q,i}\}_{i=1}^{n_q}$ such that $\cup_{i=1}^n s_{q,i}= \{\vp_{\tau} | \tau \in \cT\}$. 
    %
    We use $i(\tau)$ to denote the index of the subset for which receiver type $\tau$ belongs, i.e. $\vp_{\tau} \in s_{q,i(\tau)}$. 
    %such that $\cup_{i=1}^{n_q} s_{q,i} = \{\vp_{\tau} | \tau \in \cT\}$. 
    %
    A partition oracle with query space $\cQ$ takes a partition query $q \in \cQ$ as input, and returns the subset $s_{q,i(\tau^*)}$.\looseness-1 
\end{definition}
%
After making a partition query, the sender can leverage the fact that the true receiver belief is contained in the returned subset to design more persuasive messaging policies. 
%
An important special case is when the sender can \emph{simulate} the response of the receiver.
% deleted below as not primary motivation
%, as is the case when, e.g., the receiver is a software agent or the sender can use a machine learning model to predict receiver behavior.
%
\begin{definition}[Simulation Oracles and Simulation Queries]\label{def:sim}
    A simulation query is a tuple $q := (\sigma_q, m_q)$, where $\sigma_q : \Omega \rightarrow \cA$ is a messaging policy mapping states to actions, and $m_q \in \cA$ is a message. 
    %
    A simulation oracle takes a simulation query $q$ as input, and returns the (true) receiver type $\tau^*$'s best-response 
    %
    \begin{equation*}
        a_{q,\tau^*} = \arg\max_{a \in \cA} \mathbb{E}_{\omega \sim \vp_{\tau^*}}[u_R(\omega, a) | m_q].
    \end{equation*}
    %$a_{q,\tau^*} = \arg\max_{a \in \cA} $ $\mathbb{E}_{\omega \sim \vp_{\tau^*}}[u_R(\omega, a) | m_q]$.\looseness-1 
    %
\end{definition}

\noindent A simulation oracle is a partition oracle with a restricted set of allowable queries $\cQ\subset \cS$, where $\cS$ is the power set of receiver beliefs $\{\vp_{\tau} | \tau \in \cT\}$. 
%
The structure of a simulation oracle's query space is discussed in Theorem~\ref{fact:sep}.
%
%We explore the power of simulation queries in~\Cref{sec:helps}. 
%
%In~\Cref{sec:adaptive} and~\Cref{sec:non-adaptive}, we consider settings in which the sender can make multiple queries to the oracle. 
%
We primarily consider the setting in which the sender can make $K > 0$ costless oracle queries, although we also extend our results to the setting in which the sender can make unlimited queries, but each query $q \in \cQ$ has an associated cost $c_q \in \mathbb{R}$. 
%
Under this \emph{costly} setting the sender's goal is to maximize her Bayesian-expected utility, \emph{minus the total cost of querying}. 
%
We posit that the sender does not observe the state until \emph{after} the messaging policy is computed.
%
%This is because we do not wish to endow the sender any additional commitment power compared to the standard formulations of BP. 
%
%If the queries the sender makes to the oracle were to depend on the state, then the sender would also need to commit to the process which decides these queries. 
%
%We briefly explore this setting in~\Cref{sec:committing}.\looseness-1
We relax this assumption in~\Cref{sec:committing}.\looseness-1

The sender interacts with the oracle according to a \emph{querying policy}, as defined below. 
%As we will see, the order of the interaction matters when the sender can make multiple queries. 
%
%Two natural ways in which the sender can interact with the oracle are via
Two natural interaction regimes are 
\emph{adaptive} and \emph{non-adaptive}. %querying policies. 
%
%When the sender is querying according to 
An adaptive querying policy makes a query, observes the realized partition of the belief space, and repeats.
%then repeats until she has no queries remaining. 
%
%In contrast when using a non-adaptive querying policy, the sender must 
A non-adaptive querying policy
specifies all $K$ queries \emph{up front}, before observing the oracle's response to any of them.
%
\begin{definition}[Querying Policy]\label{def:adaptive}
    An \emph{adaptive} querying policy $\pi \; : \; \cS \times \mathbb{N} \rightarrow \cQ$ is a mapping from belief subsets and number of queries left to queries. 
    %
    A \emph{non-adaptive} querying policy $\pi \; : \; \mathbb{N} \rightarrow \cQ^*$ is a mapping from a number of queries to a set of queries.
\end{definition}
%
\begin{figure}[t]
    \centering
    \noindent \fbox{\parbox{0.9\textwidth}{
    \vspace{0.1cm}
    \textbf{Protocol: Bayesian Persuasion with Oracle Queries}
    
    \vspace{-0.3cm}
    %\noindent\rule{15.9cm}{0.4pt}
    %\noindent\rule{14.9cm}{0.4pt}
    \noindent\rule{12.5cm}{0.4pt}\vspace{1mm}
    %
    \begin{enumerate}
        %\setcounter{enumi}{-1}
        \item Sender makes $K$ oracle queries, either adaptively or non-adaptively.
        %
        \item Sender \emph{commits} to messaging policy $\sigma : \Omega \rightarrow \cM$.
        %
        \item Sender observes state $\omega \sim \vp_{\tau^*}$, where
        $\tau^* \sim \cP$ is the true receiver type.
        %
        \item Sender sends message $m \sim \sigma(\omega)$, receiver forms posterior 
        $\rbr{\vp_{\tau^*} \mid m, \sigma}$.
        %
        \item Receiver takes action $\arg\max_{a \in \cA} \mathbb{E}_{\omega \sim \vp_{\tau^*}}\sbr{u_R(\omega, a) \mid  m, \sigma}$.
    \end{enumerate}
    }}
    \caption{Summary of our setting.}
    \label{fig:our-model}
\end{figure}
%
The timing of the game is summarized in~\Cref{fig:our-model}.
% for a summary of the model we consider. 
%
The sender's goal is to compute a querying policy (either adaptive or non-adaptive, depending on the setting) that will maximize the expected sender utility obtained from the optimal messaging policy 
%that maximizes the sender utility given 
for the (endogenous) prior over receiver beliefs, i.e., the sender's objective is
%
\begin{equation*}
\max_{\pi}\mathbb{E}_{\tau\sim\cP_\pi(\cT)}\left[\max_{\sigma_{s(\tau)}} \mathbb{E}_{\omega\sim p_\tau, m \sim \sigma_{s(\tau)}(\omega)}[u_S(\omega, a(m))]\right],
\end{equation*}
%
%$\max_{\pi}\mathbb{E}_{\tau\sim\cP_\pi(\cT)}\left[\max_{\sigma_{s(\tau)}} \mathbb{E}_{\omega\sim p_\tau, m \sim \sigma_{s(\tau)}(\omega)}[u_S(\omega, a(m))]\right]$,
%$\max_{\pi,\sigma} \mathbb{E}_{\tau\sim\cP_\pi(\cT),\omega\sim p_\tau, m \sim \sigma(\omega)}[u_S(\omega, a(m))]$
%
where $P_\pi(\cT)$ is the sender's expected posterior belief over the type given the  querying policy $\pi$, $s(\tau)$ is the belief partition for which receiver type $\tau$ belongs after querying, and $a(m)$ is the action that maximizes the receiver's expected utility over her posterior given messaging policy $\sigma$ and message $m$.\looseness-1
%which enables them to design a maximally persuasive messaging policy for the true receiver belief. 

==> paper/main_body/model-v2.tex <==
\section{Model}\label{sec:setting}
%
%We first overview the Bayesian Persuasion setting in~\Cref{sec:bp}, before introducing the receiver-informed oracle in~\Cref{sec:model}.  
%
We study a Bayesian persuasion game with an informed receiver \textcolor{red}{[NSI: see \cite{kolotilin2017persuasion} which also has binary actions but continuous state and linear utilities, plus the type is indep of the state; we should figure out how to compare to this}.  There is a binary state of the world $\omega\in\Omega=\{0,1\}$. The receiver has a private signal about the state $s\in\mathcal{S}$.  
The receiver can take one of two actions $a\in\cA=\{0,1\}$.  Sender and receiver utilities are given by utility functions $u_S : \Omega \times \cA \rightarrow \mathbb{R}$ and $u_R : \Omega \times \cA \rightarrow \mathbb{R}$ respectively. We assume the sender's utility is state-independent and positive only if the receiver takes the action $a=1$, i.e., $u_S(\omega,a)=a$.
For the receiver's utility, we assume only that the receiver prefers action $a = \omega$ to action $a \neq \omega$: $u_R(1,1) \geq u_R(1,0)$ and $u_R(0,0) \geq u_R(0,1)$.  Write $\cU$ for the set of all such receiver utility functions.  
%The receiver's utility function is drawn from a distribution $G$ over $\cU$.
%The receiver's utility depends on whether the action matches the state, i.e., $u_R(\omega,a)=\mathbf{1}(a=\omega)$.\footnote{We note this form of utility function is without loss of generality in our binary state/action setting so long as the sender's utility is state-independent. \textcolor{red}{[NSI: you agree, right?]}\textcolor{blue}{[Yes, in the sense that for cases that aren't equivalent to this (e.g., fully aligned or fully misaligned), the problem is trivial/uninteresting.  So maybe also say ``...and the receiver's preferred action is state-dependent" or something like that?]}} 
The state, signal, and receiver utility function are drawn from a joint distribution $F$ over $\Omega \times \cS \times \cU$.  We assume that $F$ has finite support, and write $T$ for the number of pairs $(s,u_R)$ such that $(\omega,s,u_R)$ is in the support of $F$ for some value of $\omega$.\footnote{Some of our approximation results extend to continuous distributions over signals and receiver utilities, as we discuss in Section~\ref{sec:equil.approx}.} Given $s \in \mathcal{S}$ and $u_R \in \cU$, we write $F|_{s,u_R}$ for the marginal distribution over $\omega$ given $s$ and $u_R$.
The joint distribution $F$ and the sender's utility function $u_S$ are known to both the sender and the receiver; the signal $s$ and the receiver's utility function $u_R$ are known only to the receiver.

The sender commits to a messaging policy that maps states to messages.
%
\begin{definition}[Messaging Policy]\label{def:messaging}
    The sender's \emph{messaging policy} $\sigma : \Omega \rightarrow \cM$ is a (randomized) mapping from states to \emph{messages} $m\in\cM$.  
\end{definition}
%
\noindent We will sometimes write $\sigma(m|\omega)$ to denote $\Pr[\sigma(\omega)=m]$ and $m \sim \sigma(\omega)$ to denote a message sampled from $\sigma$ when the state is $\omega \in \Omega$.

We depart from prior formulations of this problem in our assumption that the sender has access to a simulation oracle.  This oracle simulates the receiver's optimal actions and thus yields information about the receiver's signal, $s$, and utility function, $u_R$, which helps the sender improve its messaging policy.
%
\begin{definition}[Simulation Oracle]\label{def:sim}
    A simulation oracle inputs a query $q\in\mathcal{Q}$ consisting of a tuple $(\sigma_q, m_q)$, where $\sigma_q$ is a messaging policy and $m_q \in \cA$ is a message. 
    %
    The oracle returns the receiver's  best-response given the joint distribution $F$, private signal $s$, and utility function $u_R$, i.e., it returns $a_q$ where: 
    %
    \begin{equation*}
        a_{q} = \arg\max_{a \in \cA} \mathbb{E}_{\omega}[u_R(\omega, a) | m_q,s].
    \end{equation*}
    %$a_{q,\tau^*} = \arg\max_{a \in \cA} $ $\mathbb{E}_{\omega \sim \vp_{\tau^*}}[u_R(\omega, a) | m_q]$.\looseness-1 
    %
\end{definition}
%
\noindent We assume the sender can make up to $K$ queries\footnote{We explore a model in which each query has an associated cost in Section~\ref{sec:extension.costs}; the results are largely unchanged.} and can do so adaptively.  That is, the sender can sequentially make queries, choosing each next query based on the responses to the previous queries.  Formally, a \emph{history} is a finite (possibly empty) sequence of query-action pairs.  We write $\mathcal{H}$ for the set of all histories.  We denote the sender's querying policy by the function $\pi \colon \mathcal{H} \to \mathcal{Q}$ that maps a sequence of past queries and responses to a next query.  We will also abuse notation and write $\pi(s,u_R)$ to denote the history generated by the application of $\pi$ until its termination given the receiver's signal and utility function.

\begin{figure}[t]
    \centering
    \noindent \fbox{\parbox{0.89\textwidth}{
    \textbf{Protocol: Bayesian Persuasion with Oracle Queries}
    \begin{enumerate}
    \item the sender uses query policy $\pi$ to query the simulation oracle up to $K$ times, resulting in query history $H$;
    \item the sender commits to a messaging policy $\sigma_H$, which is visible to the receiver; 
    \item the state $\omega$ is revealed privately to the sender; 
    \item the message $m \sim \sigma_H(\omega)$ is sent to the receiver;
    \item the receiver chooses an action $a = a(m) \in\cA$.  
    \end{enumerate}
    }}
    \caption{Summary of our setting.}
    \label{fig:our-model}
\end{figure}

The timing of the game is summarized in \Cref{fig:our-model}.
%
We study perfect Bayesian equilibria (PBE) of this game.  In our game, a strategy for the sender is a query policy $\pi$, plus a messaging policy rule $\sigma$ that maps potential query histories to messaging policies (where we write $\sigma_H$ for the messaging policy corresponding to query history $H$).  A strategy for the receiver is an action rule $a \colon \mathcal{M} \times \mathcal{S} \times \cU \to \mathcal{A}$ mapping a message, signal, and utility function to an action.

\begin{definition}
    A profile of strategies $(\pi^*, \sigma^*, a^*)$, together with a belief rule $B_S \colon \mathcal{H} \to \Delta(\mathcal{S} \times \cU)$ for the sender mapping query histories to distributions over receiver signals and utilities, plus a belief rule $B_R \colon \mathcal{M} \times \mathcal{S} \times \cU \to \Delta(\Omega)$ for the receiver mapping messages, signals, and utility functions to distributions over the state of the world, is a perfect Bayesian equilibrium if:
\end{definition}
%\textcolor{red}{[NSI: todo, define me]}
\begin{enumerate}
    \item For each $m \in \mathcal{M}$, $s \in \mathcal{S}$, and $u_R \in \cU$, action $a^*(m, s, u_R)$ maximizes the receiver's expected utility given belief $B_R(m, s)$:
    \[ a^*(m) \in \arg\max_a \{ \mathbb{E}_{\omega \sim B_R(m, s)}[ u_R( \omega, a) ] \} \]
    \item Belief $B_R(m,s,u_R)$ is the correct posterior distribution over $\omega$ given $s$, $u_R$, $\sigma^*_H$, and the fact that $\sigma^*_H(\omega) = m$.\footnote{It is possible that some tuples $(m,s,u_R)$ may have probability $0$, in which case $B_R(m,s,u_R)$ can be arbitrary.  We note that since $m$ is generated according to $\sigma^*_H$, which is known to the receiver, tuples $(m,s,u_R)$ of probability $0$ cannot occur even off the equilibrium path of play.}
    \item For each $H \in \mathcal{H}$, messaging policy $\sigma^*_H$ maximizes the sender's expected utility given belief $B_S(H)$:
    \[ \sigma^*_H \in \arg\max_{\sigma} \{ \mathbb{E}_{(s,u_R) \sim B_S(H), \omega \sim F|_{s,u_R}}[ u_S( \omega, a^*(\sigma(\omega), s, u_R) ) ] \]
    \item Belief $B_S(H)$ is a correct posterior distribution over $(s, u_R)$, given $\pi^*$ and the fact that $\pi^*$ generates history $H$.
    \item Sender's query policy $\pi^*$ maximizes the sender's expected utility given $\sigma^*$ and $a^*$:
    \[ \pi^* \in \arg\max_{\pi} \{ \mathbb{E}_{(\omega,s,u_R) \sim F, H \sim \pi }[ u_S( \omega, a^*(\sigma^*_H(\omega), s, u_R) ) ] \} \]
\end{enumerate}

A few notes are in order.  We also emphasize that the state $\omega$ is revealed to the sender only after the messaging policy $\sigma_H$ is announced, so in particular the query history has no dependency on $\omega$ after conditioning on $s$ and $u_R$.  In particular, this means that since the messaging policy $\sigma^*_H$ is observable by the receiver, the query history $H$ has no further bearing on the receiver's beliefs, utility, or choice of action.

We also note that optimality of the query policy $\pi^*$ implies that, given any \emph{partial} history $H$ of fewer than $K$ queries, the subsequently chosen query $\pi^*(H)$ must also be utility-optimizing for the sender given the posterior over $s$ and $u_R$ induced by $H$.  And while we do not impose the restriction explicitly, we note that since the generation of histories $H$ is mechanical given the choice of $\pi^*$ and the realization of $(s, u_R)$, any history $H$ that is inconsistent with any realization of $(s, u_R)$ will have probability $0$ of being observed, even off the equilibrium path of play.

Finally, we note that we assumed the receiver has a private signal correlated with the state and thus knows something about the state that the sender does not at the beginning of the game.  This (rather standard) setting is sometimes motivated by scenarios where the receiver might have access to news that the sender does not have access to when designing her messaging policy.  It can be interesting to consider what happens if the receiver has ``fake'' news but acts as if her news is true. One way to model this is to assume that two pairs of world state and signal are drawn independently from $F$ given $u_R$, say $(\omega,s), (\omega',s') \sim F|_{u_R}$, where $\omega$ is the true state but the receiver observes signal $s'$ and (incorrectly) infers that $\omega$ is distributed as $F|_{s',u_R}$.  All our results carry through to this setting with minor modifications to the algorithms. 
%\textcolor{red}{[NSI: Brendan, can you rewrite the model in the next-to-last sentence to jive better with the signal language we're now using?  and/or put this later on where we're already talking about beliefs?]}\textcolor{blue}{[BJL: Done]}



\iffalse
%
When the sender and receiver share a common prior $\vp$ it is without loss of generality to message according to the set of possible actions (i.e. $\cM = \cA$) via a revelation principle-style argument. (See~\cite{kamenica2011bayesian} for more details.)
%
Under this setting, a message has the interpretation of being the action that the sender is recommending the receiver to take. 
%
We say that the sender's messaging policy is \emph{Bayesian incentive-compatible} (BIC) if it is always in the receiver's best interest to follow the sender's action recommendations.\looseness-1 
%
\begin{definition}[Bayesian Incentive-Compatibility]\label{def:BIC}
    A messaging policy $\sigma : \Omega \rightarrow \cA$ is Bayesian incentive-compatible if for every action $a \in \cA$,
    %
    \begin{equation*}
        \mathbb{E}_{\omega \sim \vp}[u_R(\omega, m) | m] \geq \mathbb{E}_{\omega \sim \vp}[u_R(\omega, a) | m].
    \end{equation*}
    %
    %$\mathbb{E}_{\omega \sim \vp}[u_R(\omega, m) | m] \geq \mathbb{E}_{\omega \sim \vp}[u_R(\omega, a) | m]$. 
    %
    We assume that if the receiver is indifferent between two actions, she breaks ties in favor of the sender's recommended action.\looseness-1 
    %
\end{definition}  
%
\noindent The sender's optimal messaging policy $\sigma$ is given by the solution to the following linear program:
%
\begin{equation*}
\begin{aligned}
    \max_{\sigma} \; &\mathbb{E}_{\omega \sim \vp, m \sim \sigma(\omega)}[u_S(\omega, m)]\\
    %
    \text{ s.t. } \;\; \mathbb{E}_{\omega \sim \vp}[u_R(\omega, m) | m, \sigma] &\geq \mathbb{E}_{\omega \sim \vp}[u_R(\omega, a) | m, \sigma], \;\; \forall a \in \cA, m \in \cM
\end{aligned}
\end{equation*}
%
The time it takes to compute the optimal messaging policy is $\mathcal{O}(\lp(dA, A^2 + dA))$, where $\lp(x,y)$ is the time it takes to solve a linear program with $x$ variables and $y$ constraints. 
%
Some of our results are specialized to the following \emph{binary} setting, which is itself a popular model of persuasion (see, e.g. \cite{parakhonyak2022persuasion, kosterina2022persuasion, hu2021robust, kolotilin2017persuasion} for various versions of this setting studied in the literature).\looseness-1
%
\begin{definition}[Binary Bayesian Persuasion]\label{def:bin}
    In the Binary Bayesian Persuasion setting, $\omega \in \{0, 1\}$, $a \in \{0, 1\}$, and the prior over states can be described by a single number $p := \mathbb{P}(\omega = 1)$. 
    %
    Furthermore, we assume the following utility functions for the sender and receiver: 
    \begin{equation*}
    \begin{aligned}
        u_S(\omega, a) = \mathbbm{1}\{\omega = 1\}, \;\;\;
        %
        u_R(\omega, a) = \mathbbm{1}\{\omega = a\}
    \end{aligned}
    \end{equation*}
    %$u_S(\omega, a) = \mathbbm{1}\{\omega = 1\}$, $u_R(\omega, a) = \mathbbm{1}\{\omega = a\}$. 
    %
    In other words, the sender always wants to incentivize the receiver to take action $a=1$, but the receiver only wants to take action $a=1$ whenever $\omega = 1$.
\end{definition}
\fi

==> paper/main_body/non-adaptive_qp.tex <==
\section{Non-Adaptive Querying Policies}\label{sec:non-adaptive}
%
When querying non-adaptively, the sender must make all $K$ queries \emph{up front} (recall~\Cref{def:adaptive}). 
%
Our results in this setting differ significantly between Binary BP with simulation queries and the general setting. 
%
The following notion of a \emph{non-adaptive belief partition} will be useful later on.\looseness-1 
%
\begin{definition}[Non-Adaptive Belief Partition]\label{def:partition}
    %
    A set of non-adaptive queries $\cQ' \subseteq \cQ$ induces a partition $H_{\cQ'}$ over receiver belief space such that $\bigcup_{\eta \in H_{\cQ'}} \eta = \{\vp_{\tau} | \tau \in \cT\}$. 
    %
    Receiver belief $\vp_{\tau}$ belongs to the subset $\eta_{\cQ'}[\tau] \in H_{\cQ'}$ such that $\eta_{\cQ'}[\tau] := \bigcap_{q \in \cQ'} s_{q,i(\tau)}$.
    %
\end{definition}
%
%The key difference between~\Cref{def:partition} and \Cref{def:feasible} is that in the non-adaptive setting, the sender does not get to see the outcome of a query until all queries are made. 
%
\subsection{Computing Non-Adaptive Querying Policies}\label{sec:na-computing}
%
%\subsubsection{Optimal Solution for the Binary Setting}\label{sec:bin-computing}
%
%
\begin{figure}[th]
    \centering
    \includegraphics[width=\textwidth]{figures/bin-dp.png}
    \caption{Sender's expected utility $u(i')$ (y-axis) as a function of the cutoff receiver index $i'$ in Binary BP. Under this problem instance there are five types with beliefs $p_1 = 0.5$, $p_2 = 0.4$, $p_3 = 0.3$, $p_4 = 0.2$, and $p_5 = 0.1$ (x-axis), and second-order prior $\cP(\tau_1) = 0.2$, $\cP(\tau_2) = 0.01$, $\cP(\tau_3) = 0.39$, $\cP(\tau_4) = 0.2$, and $\cP(\tau_5) = 0.2$. 
    %
    (Recall the form of the optimal messaging policy in~\Cref{cor:opt-binary}.)
    %
    Blue: Sender's utility as a function of the cutoff index when they make no queries. 
    %
    The sender's optimal utility is given by the blue dashed line. 
    %
    Red: Sender's utility as a function of cutoff index when they make the simulation query $q$ which separates $\{\tau_1, \tau_2, \tau_3\}$ from $\{\tau_4, \tau_5\}$. 
    %
    The red dashed line denotes the sender's utility from messaging optimally after making query $q$.
    %https://www.desmos.com/calculator/hdun0wsdk3
    }
    \label{fig:bin-dp}
\end{figure}
%
We find that the optimal non-adaptive querying policy may be computed via dynamic programming when considering simulation queries in Binary BP. 
%
However unlike in the adaptive setting, the optimal querying policy is computed by leveraging the fact that there is a ``total ordering'' over receiver beliefs when there are two states, and iteratively building solutions for larger sets of receivers. 
%
We overload notation and use $q$ to index the receiver belief with the smallest prior which takes action $a=1$ in response to simulation query $q \in \cQ$. 
%
Given a set of $T$ receiver types $\{1, \ldots, T\}$ where $p_1 > p_2 > \cdots > p_T$, \Cref{alg:dp-na} keeps track of the optimal sender utility achievable with $k$ queries when in receiver subset $\{1, \ldots, i\}$ for all $1 \leq i \leq T$. 
%
Due to the structure induced by non-adaptivity in this setting, we are able to write the sender's expected utility for $k+1$ queries in receiver subset $\{1, \ldots, i+1\}$ as a function of the optimal solution for $k$ queries in subset $\{1, \ldots, i\}$.
%
See~\Cref{fig:bin-dp} for a visualization of the sender's expected utility in Binary BP.\looseness-1 
%
\begin{algorithm}[t]
\caption{Computing the Optimal Non-Adaptive Querying Policy: Binary BP, $K$ Queries}\label{alg:dp-na}
\begin{algorithmic}
\Require Query budget $K \in \mathbb{N}$\\
%
\begin{itemize}
    %
    \item Set 
    %
    \begin{equation*}
        V[i, j, 0] := \sum_{l=q}^i \cP(\tau_l) \cdot \mathbb{E}_{\tau \sim \cP(i,j)} \mathbb{E}_{\omega \sim \vp_{\tau}} \mathbb{E}_{m \sim \sigma^*_{\cP(i,j)}(\omega)} u_S(\omega, m)
    \end{equation*}
    %
    %$V[i, j, 0] := \sum_{l=q}^i \cP(\tau_l) \cdot \mathbb{E}_{\tau \sim \cP(i,j)} \mathbb{E}_{\omega \sim \vp_{\tau}} \mathbb{E}_{m \sim \sigma^*_{\cP(i,j)}(\omega)} u_S(\omega, m)$
    %
    for all $1 \leq i \leq j \leq T$, where $\sigma^*_{\cP(i,j)}$ is the optimal messaging policy of~\Cref{cor:opt-binary} under second-order prior $\cP(i,j)$, and $i,j$ is shorthand for types $\{i, \ldots, j\}$. 
    %
    \item For every $1 \leq k \leq K$ and $1 \leq j \leq T$, compute 
    %
    \begin{equation*}
        V[1, j, k] := \max_{q \in \cQ} V[q+1, j, 0] + V[1, q, k-1]
    \end{equation*}
    %
    %$V[1, j, k] := \max_{q \in \cQ} V[q+1, j, 0] + V[1, q, k-1]$ 
    %
    \item The optimal policy then makes the $K$ queries which obtain value $V[1, T, K]$.\looseness-1
\end{itemize}
%
\end{algorithmic}
\end{algorithm}
%
\begin{restatable}{theorem}{DPna}
\label{thm:DP-na}
    In Binary BP with simulation queries,~\Cref{alg:dp-na} computes the sender's optimal non-adaptive querying policy in $\mathcal{O}(T^3K)$ time.
\end{restatable}
%

%
%\subsubsection{Hardness Result for the General Setting}\label{sec:hardness}
%
\Cref{alg:dp-na} may be used to compute the optimal non-adaptive querying policy for the costly setting by (1) setting $K=T-1$ (2) introducing a new query $q_{\varnothing}$ such that $c_{q_{\varnothing}} = 0$, and using the following modified update step:
%
\begin{equation*}
    V[1, j, k] := \max_{q \in \cQ} V[q+1, j, 0] + V[1, q, k-1] - c_q.
\end{equation*}
%
\begin{corollary}
    In the Binary BP setting with costly simulation queries, the above modification to~\Cref{alg:dp-na} computes the sender's non-adaptive querying policy in $\mathcal{O}(T^3K)$ time. 
\end{corollary}

%
The key idea behind~\Cref{alg:dp-na} is that in Binary BP with simulation queries, there is always a ``total ordering'' over both receiver beliefs and queries, and thus one can use dynamic programming in order to iteratively construct an optimal solution. 
%
This intuition does not carry over to the setting with general partition queries, as no such total ordering exists. 
%
In fact, the corresponding decision problem is NP-Complete.\looseness-1 
%
\begin{definition}[Non-Adaptive Decision Problem]\label{def:nadp}
    Given $(\cT, \cP, \cQ, K, u)$ where $\cT$ is a set of receiver types, $\cP$ is a second-order prior over receiver types, $\cQ$ is a set of allowable queries, $K \in \mathbb{N}$, and $u \in \mathbb{R}_+$, does there exist a collection of queries $\cQ' \subseteq \cQ$ of size $|\cQ'| \leq K$ such that the sender can achieve expected utility at least $u$ after making queries $\cQ'$?
\end{definition}
%
\begin{restatable}{theorem}{hardness}
\label{thm:hardness}
    The Non-Adaptive Decision Problem is NP-Complete in Binary BP.\looseness-1
\end{restatable}
%
To prove NP-Hardness, we reduce from Set Cover. 
%
Given a universe of elements $U$, a collection of subsets $S$, and a number $K$, the set cover decision problem asks if there exists a set of subsets $S' \subseteq S$ such that $|S'| \leq K$ and $\bigcup_{s \in S'} s = U$. 
%
Our reduction proceeds by creating a receiver type for every element in $U$ and a partition query for every subset in $S$. 
%
We set $u$ and $\{p_{\tau}\}_{\tau \in \cT}$ in such a way that the sender can only achieve expected utility $u$ if she can distinguish between every receiver type using $K$ non-adaptive queries, i.e. the receiver subset for type $\tau$ is a singleton for all $\tau \in \cT$. 
%
Finally, we show that under this construction the answer to the set cover decision problem is $\texttt{yes}$ if and only if the answer to the corresponding non-adaptive decision problem is also $\texttt{yes}$. 
%
\subsection{Properties of the Sender's Utility}\label{sec:properties}
%
Motivated by the hardness result of~\Cref{sec:na-computing}, we examine how the sender's expected utility changes as a function of the queries she makes. 
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig-submod.png}
    \caption{Submodularity in Binary BP with simulation queries. 
    %
    Under this problem instance there are five types with beliefs $p_1 = 0.5$, $p_2 = 0.4$, $p_3 = 0.3$, $p_4 = 0.2$, and $p_5 = 0.1$ (x-axis), and second-order prior $\cP(\tau_1) = 0.2$, $\cP(\tau_2) = 0.01$, $\cP(\tau_3) = 0.39$, $\cP(\tau_4) = 0.2$, and $\cP(\tau_5) = 0.2$. 
    %
    (Recall the form of the optimal messaging policy in~\Cref{cor:opt-binary}.)
    %
    Blue: Sender's utility as a function of the cutoff index. 
    %
    Red: Sender's utility as a function of cutoff index when they know the true receiver belief is either $p_2$, $p_3$, or $p_4$ from previous queries. 
    %
    Blue and red crosses denote the sender's expected utility after query $q$ is made. 
    %
    The black cross denotes both a blue and red cross on top of one another. 
    %
    The blue and red dashed lines denote the sender's respective marginal gains in utility from messaging optimally after making query $q$. 
    %
    The marginal gain is always higher when the sender has more uncertainty over the receiver's true type. 
    %see desmos.com
    }
    \label{fig:submod}
\end{figure}
%
%
%We begin by showing that the sender gets \emph{decreasing marginal utility} for making additional simulation queries in Binary BP. 
%
%As a corollary, this implies that the greedy querying policy is approximately optimal under this setting. 
%
%In contrast, we show that decreasing marginal utility of queries does \emph{not} hold in the general setting. 
%
%\subsubsection{Decreasing Marginal Gains in the Binary Setting}\label{sec:bin-marginal}
%
\begin{restatable}{theorem}{submod}
\label{thm:submod}
    %
    In Binary BP, the sender's Bayesian-expected utility exhibits decreasing marginal returns from additional simulation queries. 
    %
\end{restatable}
%
The proof proceeds via a case-by-case analysis on the difference in expected sender utility as a function of the queries which are made. 
%
The key step is to leverage the form of the sender's optimal messaging policy under uncertainty in Binary BP (\Cref{cor:opt-binary}) to argue that no matter how an additional query splits the current belief partition, the expected marginal gain is always weakly larger than whenever the set of queries is a superset. 
%
See~\Cref{fig:submod} for a visualization of this idea.\looseness-1
%
\begin{algorithm}[t]
\SetAlgoNoLine
%
\caption{Non-Adaptive Greedy Querying Policy}\label{alg:greedy}
%
\KwIn{Query budget $K \in \mathbb{N}$}
%
Set $\cQ_0 = \emptyset$
%
\For{$j = 0, 1, \ldots, K-1$}
{
    Add query 
    %
    \begin{equation*}
        x_{j+1} = \arg\max_{q \in \cQ} \mathbb{E}_{\tau \sim \cP}\mathbb{E}_{\omega \sim \vp_{\tau}}\mathbb{E}_{m \sim \sigma_{\cP(\eta_{\cQ_j \cup q)}[\tau]}(\omega)}[u_S(\omega, m)] %- \mathbb{E}_{p \sim \cP}\mathbb{E}_{\omega \sim p}\mathbb{E}_{m \sim \sigma_{\eta_i(p)}(\omega)}[u_S(\omega, m)]
    \end{equation*}
    %
    Set $\cQ_{j+1} \leftarrow \cQ_{j} \cup \{x_{j+1}\}$
}
%
\Return $\cQ_K$
%
\end{algorithm}
%

An immediate corollary of~\Cref{thm:submod} is that the greedy non-adaptive querying policy (\Cref{alg:greedy}) is $(1 - 1/e)$-approximately optimal in Binary BP. 
%
\begin{restatable}{corollary}{greedyperformance}\label{thm:greedy-approx}
    In the Binary BP setting, the non-adaptive querying policy $\cQ_K$ produced by~\Cref{alg:greedy} is a $(1-1/e)$-approximation of $\cQ_K^*$ and can be computed in time $\mathcal{O}(T^4)$.
    %
    \iffalse
    \begin{equation*}
    \begin{aligned}
        &\mathbb{E}_{p \sim \cP} \mathbb{E}_{\omega \sim p} \mathbb{E}_{m \sim \sigma_{\gamma_{k}(p)}(\omega)}[u_S(\omega, m)] - \mathbb{E}_{p \sim \cP} \mathbb{E}_{\omega \sim p} \mathbb{E}_{m \sim \sigma_{\cP}(\omega)}[u_S(\omega, m)]\\
        %
        \geq &(1 - 1/e) \cdot (\mathbb{E}_{p \sim \cP} \mathbb{E}_{\omega \sim p} \mathbb{E}_{m \sim \sigma_{\gamma^*(p)}(\omega)}[u_S(\omega, m)] - \mathbb{E}_{p \sim \cP} \mathbb{E}_{\omega \sim p} \mathbb{E}_{m \sim \sigma_{\cP}(\omega)}[u_S(\omega, m)])
    \end{aligned}
    \end{equation*}
    \fi 
    %
\end{restatable}

%
All of our results for Binary BP carry over to the non-adaptive variant of the costly (simulation) query setting. 
%
In particular, in~\Cref{app:greedy-costly-bin} we show that the sender's expected utility still exhibits decreasing marginal returns in the costly Binary BP setting, and a natural modification of the non-adaptive greedy policy (\Cref{alg:costly-greedy}) is $(1 - 1/e)$-approximately optimal. 
%

However, the above properties do not extend to the sender's expected utility in the general setting. 
%
%
\begin{figure}[th]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/bad_ex.png}
    \caption{Illustration of~\Cref{ex:greedy-bad2} in two dimensions. 
    %
    Under this setting, there are four receiver types $\tau_1$, $\tau_2$, $\tau_3$, $\tau_4$ and two queries. 
    %
    Query $q_1$ separates $\tau_1$ and $\tau_3$ from $\tau_2$ and $\tau_4$. 
    %
    Query $q_2$ separates $\tau_1$ and $\tau_2$ from $\tau_3$ and $\tau_4$. 
    %
    The sender and receiver utilities are constructed in such a way that the sender's expected utility only increases after making both $q_1$ and $q_2$.}
    \label{fig:bad-ex}
\end{figure}
%
Consider the following example:\looseness-1
%
\begin{example}\label{ex:greedy-bad2}
%
For some $L \in \mathbb{N}$, consider a setting with state space $\Omega = \{\omega_0, \omega_1, \ldots, \omega_{2^L - 1}, \omega_{\varnothing}\}$ and receiver types $\cT = \{0, 1, \ldots, 2^L - 1 \}$ where receiver $\tau_i$ has prior $\vp_i$ such that $\vp_i[\omega_{\varnothing}] = \epsilon$ for some $\epsilon > 0$, $\vp_i[\omega_j] = \frac{\epsilon}{2}$ for all $j \neq i$, which implies that $\vp_i[\omega_i] = 1 - (\frac{1}{2} \cdot 2^L + 1) \cdot \epsilon$.  
%
Suppose that the set of receiver actions is equal to the set of states, i.e. $\cA = \Omega$. 
%
Consider the sender utility function 
%
\begin{equation*}
    u_S(\omega, a) = \mathbbm{1}\{a \neq \omega_{\varnothing}\}
\end{equation*}
%
%$u_S(\omega, a) = \mathbbm{1}\{a \neq \omega_{\varnothing}\}$ 
%
and let %$u_R(\omega, a) = 2 \cdot \mathbbm{1}\{a = \omega\} - 1$ if $a \in \Omega \backslash \{\omega_{\varnothing}\}$ and $u_R(\omega, \omega_{\varnothing}) = 0$. 
%
\begin{equation*}
    u_R(\omega, a) = 
         \begin{cases}
             2 \cdot \mathbbm{1}\{a = \omega\} - 1 \;\; &  \;\; \text{if } a \in \Omega \backslash \{\omega_{\varnothing}\}\\
             %
             0 \;\; & \;\; \text{if } a = \omega_{\varnothing}.
         \end{cases}
\end{equation*}
%
Suppose there are $L$ queries $\cQ = \{q_1, \ldots, q_L\}$, where query $q_j$ reveals the $j$-th bit of $\vp_{i^*}$, where $i^*$ is the true receiver type.  
%
Finally, let $\cP$ be the uniform distribution over $\cT$.
%
\end{example}
%
See~\Cref{fig:bad-ex} for an illustration of this setting when $L=2$. 
%
The receiver's actions can be interpreted as ``guesses'' as to what the underlying state is: she gets utility $1$ if she correctly guesses the state and utility $-1$ if she makes an incorrect guess. 
%
The receiver always gets utility $0$ if she guesses that the state is $\omega_{\varnothing}$, regardless of whether this guess is correct. 
%
The sender's utility is such that she wants to incentivize the receiver to guess any state other than $\omega_{\varnothing}$. 
%
If the sender knows the receiver's belief exactly, she can incentivize her to \emph{never} guess $\omega_{\varnothing}$. 
%
However if the sender has \emph{any} uncertainty over the receiver's belief, the receiver will guess $\omega_{\varnothing}$ with (the same) constant probability under the sender's optimal messaging policy, regardless of how much uncertainty the sender has. 
%
\begin{restatable}{theorem}{notsubmod}\label{thm:not-submod}
    Consider the setting of~\Cref{ex:greedy-bad2} with $\epsilon = \frac{1}{2^{L-1} + 2}$. The sender's Bayesian-expected utility does not exhibit decreasing marginal returns from additional queries. 
    %
\end{restatable}
%
The proof proceeds by showing that under the setting of~\Cref{ex:greedy-bad2}, it is possible to completely distinguish between all receivers with $L$ queries, but not with $L' < L$ queries. 
%
Using~\Cref{ex:greedy-bad2} as a building block, we can also construct an instance in which the greedy non-adaptive querying policy performs exponentially worse than the optimal policy (\Cref{thm:greedy-exp}).\looseness-1 

==> paper/main_body/preliminaries-v2.tex <==
\section{Preliminaries}\label{sec:think}

We begin with structural results which showcase intuition and will be useful later. We first show that any messaging policy is outcome-equivalent to one with just $T+1$ messages, where recall that $T$ is the number of distinct pairs $(s,u_R)$ that appear in the support of $F$.  We then use the underlying arguments of this proposition to derive a useful geometric property of simulation queries.  Namely, we argue that there is a total ordering over all possible receivers with respect to how easily they are persuaded to take action $a=1$, and any simulation query is equivalent to a threshold that separates receivers into those from whom this parameter is greater than some threshold and those for whom it is less.  %whose belief in state $\omega=1$ is greater than a threshold $p \in [0,1]$ and those for whom it is less than $p$.

\subsection{Optimal Persuasion Under Uncertainty}\label{sec:unknown_prior}

Our binary setting exhibits a particularly clean structure.  For any messaging policy and any message sent according to that policy, possible receivers are partitioned into two sets: those that induce action $a=1$ in response to the message and those that induce action $a=0$.  
%Furthermore, since the state is binary, 
The heterogeneity among possible receivers is driven by the receiver's belief of being in the high state $\omega=1$ and the receiver's utility function $u_R$. 
%Together these determine how a receiver will act in response to a message.  
While this variation appears multi-dimensional, we note that a message policy and a choice of message together form a signal that is correlated with the state $\omega$, and any receiver who chooses action $a=1$ given some message would also choose $a=1$ when given a message that is only more correlated with $\omega = 1$.  We can therefore associate with each possible receiver a minimally convincing message that induces the action $a=1$, which allows us to sort receivers by how easily they are convinced.
%order all possible messages (from all possible messaging policies) by their correlation with the event $\omega=1$, and find for each receiver a minimally convincing message that induces the action $a=1$. 
%single-dimensional and totally-ordered by the weight the belief places on a high state $\omega=1$. 
Therefore, the partition of beliefs induced by a message can be represented by a single threshold: receivers more easily convinced than the threshold induce the action $a=1$ and those lower induce action $a=0$.  These observations imply that the sender's optimal messaging policy has size $T+1$. 
%\textcolor{red}{[NSI: need to define $T$ in model section (and fix terminology re beliefs/types/signals/etc.), also is this intuition too repetitive with the proof itself?]} BL: I think it's okay, but let's revisit once the proof is in.

To formalize this, note first that each signal $s \in \mathcal{S}$ and receiver utility function $u_R \in \cU$ induces a distribution $F|_{s,u_R}$ over $\Omega = \{0,1\}$, which can be described by a probability $p \in [0,1]$ that $\omega = 1$.  We can therefore %equivalently describe 
associate with each possible receiver a (prior) \emph{belief} $p \in [0,1]$.  Further, if after observing the sender's message the receiver's posterior belief that $\omega = 1$ is $\beta \in [0,1]$, then the receiver will choose action $a=1$ precisely if $\beta u_R(1,1) + (1-\beta) u_R(0,1) \geq \beta u_R(1,0) + (1-\beta) u_R(0,0)$, or equivalently 
\[ \beta \geq \frac{u_R(0,0) - u_R(1,0)}{(u_R(1,1) - u_R(0,1)) + (u_R(0,0) - u_R(1,0))}. \]
We can therefore also associate with each receiver a \emph{posterior threshold} $\beta \in [0,1]$.

\textcolor{blue}{[BJL: Got to here]}

%, rather than a signal $s \in \mathcal{S}$.  We will write $\mathcal{T} \subset [0,1]$ for the set of probabilities induced by signals in $\mathcal{S}$, which we can assume without loss of generality are distinct so that $T = |\mathcal{T}|$.  
%We will sometimes refer to $\mathcal{T}$ as the set of receiver \emph{types}, 
%\textcolor{red}{[NSI: I'm worried about this terminology because CS people will think a type is a parameter in the receiver's utility function. The belief is also a parameter in the utility function but feels fundamentally different (or is it?).  We should figure this out, tell the reader which it is, and if they're different consider using $\mathcal{B}$ and ``beliefs'' as opposed to $\mathcal{T}$ and types throughout. Also Brendan/I've been using $p$ and not $\tau$ for a receiver belief (or type) but there are some carryovers of $\tau$ from previous versions]}\textcolor{blue}{[BJL: removed the reference to types here.  I've been changing $\tau$ to $p$ where I see it, but probably still missed a few.]} 
We refer to $\mathcal{T}$ as the set of receiver \emph{beliefs}, which we denote $\mathcal{T} = \{p_1, p_2, \dotsc, p_T\}$ where $p_1 > p_2 > \dotsc > p_T$, and write $\cP(p_i)$ for the probability (over the realization of signal $s$) that the receiver's belief is $p_i$.

%In the standard Bayesian persuasion framework, the receiver's beliefs are known (i.e., there is no private signal $s$).  In this case, a well-known revelation-style argument shows that, without loss of generality, the sender can use the action space as the message space (i.e. $\cM = \cA$).  When the receiver has private information, the standard arguments no longer suffice.  In principle, the sender might wish to send a menu which specifies a different action for each possible receiver belief.  Indeed, as we show in Appendix~\ref{}, this might be necessary for non-binary action spaces.  However, in the binary persuasion problem we study, $2$ messages suffice. \textcolor{red}{[NSI: this has two steps i think, first we should show that because the state is binary, we can assume wlog that the signal space is binary; then we do the revelation style thing.  If that's right, something about that should go in this paragraph (todo for Brendan after writing proof)]} \textcolor{blue}{[BJL: An alternative is to first show that any message induces a threshold of behavior in the binary setting, since if any type takes action 1 then any more-optimistic type takes action 1 as well.  This immediately implies that a message space of size $M = T + 1$ suffices (and is most of the proof of Proposition~\ref{fact:rp2}).  We'd also use it later to characterize the power of simulation queries.]}

We say two messaging policies $\sigma$ and $\sigma'$ are {\em outcome equivalent} if for all $\omega$, $m\in\sigma(\omega)$, $m'\in\sigma'(\omega)$ and receiver prior $p$, the receiver-optimal action $a$ upon seeing $m$ equals the receiver-optimal action $a'$ upon seeing $m'$. 
%\textcolor{red}{[NSI: please check]} BL: checked, looks good.
%
\textcolor{teal}{KWH: The following ``revelation principle''-style argument is well-known in the literature on persuasion with multiple receivers---we state it here for completeness.}

\begin{restatable}{proposition}{rp}\label{fact:rp2}
    In binary Bayesian persuasion, for any messaging policy $\sigma$, there is an outcome-equivalent policy $\sigma'$ with just $M = T + 1$.  Moreover, these messages can be written as $\{m_0, m_1, \dotsc, m_T\}$, where a receiver with prior $p_i$ will take action $a = 1$ upon receiving message $m_j$ if and only if $j \geq i$.
\end{restatable}
\begin{proof}
    A receiver with prior $p$ takes action $a=1$ after seeing message $m$ if and only if $p \geq \frac{\sigma(m|0)}{\sigma(m|1) + \sigma(m|0)}$.
    %
    Therefore if a receiver with prior $p$ takes action $1$ after seeing a message $m$, any receiver with belief $p' \geq p$ will also take action $a=1$.
    %
    %Similarly, a receiver with prior $p$ will take action $a=0$ after seeing message $m$ if and only if $p < \frac{\sigma(m|0)}{\sigma(m|1) + \sigma(m|0)}$, which implies that a receiver with prior $p' \leq p$ will also take action $a=0$.
    %
    There are therefore at most $T + 1$ distinct subsets of receiver beliefs that are induced to take action $a=1$ on any message $m$ of signaling policy $\sigma$, each corresponding to a minimal belief $p_i \in \mathcal{T}$ that takes the action (plus one more to denote no receiver taking the action).  
    
    Let $\sigma'$ be the messaging policy with messages $m_0, m_1, \dotsc, m_T$, such that $\sigma'(\omega) = m_i$ whenever $\sigma(\omega)$ would induce receivers with beliefs $\{p_1, \dotsc, p_i\}$ to act (or $m_0$ if it induces no receiver to act).  Then $\sigma$ and $\sigma'$ are outcome equivalent by construction, and $\sigma'$ has the required structure of $T+1$ messages.
%    \textcolor{red}{[NSI: todo]}
%    Proof has two steps:
%    \begin{enumerate}
%        \item For any message, if a receiver with prior $p$ would choose action $a = 1$, then a receiver with prior $p' > p$ would choose action $a = 1$ as well.  So for any policy $\sigma$ and message $m$ there is a threshold $\theta$ such that receivers with priors greater than $\theta$ are the ones who take action $a = 1$.
%        \item If two messages generate thresholds that don't separate any receivers, then the messages are equivalent in terms of the actions they induce.  This equivalence partitions all messages into at most $T+1$ equivalence classes.  So it suffices to use at most this many messages.
%    \end{enumerate}
\end{proof}

We note that $T+1$ messages may be necessary.  For example, suppose there are two equally-likely receiver beliefs, $\{0.25, 0.75\}$.  In this case, a messaging policy with message space $\mathcal{M} = \{m_0, m_1, m_2\}$ that uniformly randomizes between messages $m_0$ and $m_1$ when $\omega = 0$, and uniformly randomizes between messages $m_1$ and $m_2$ when $\omega = 1$, induces unique behaviors on each message.  Indeed, any receiver that receives message $m_0$ can infer that $\omega = 0$ so they choose action $a=0$, and any receiver that receives message $m_2$ can infer that $\omega = 1$ so they choose action $a = 1$.  However, upon receiving message $m_1$, an agent with belief $p_i$ will have posterior belief $p_i$ as well, so an agent of type $p_1 = 0.75$ would take action $a=1$ upon receiving message $m_1$, whereas an agent of type $p_2 = 0.25$ would not.

In Section~\ref{sec:optimal.policy} we show that there always exists a sender-optimal messaging policy that uses just $2$ messages. Nevertheless, we describe the structure of all (possibly suboptimal) message policies as it will be useful both as a stepping-stone toward that optimality characterization, and as a way to describe the geometry of simulation queries, which we explore next. %\textcolor{red}{[NSI: can we motivate why we care that $T+1$ may be necessary when at the end of the day we just need $2$? like why did we write up this prop?]}

\subsection{The Geometry of Simulation Queries}\label{sec:helps}

Another implication of the argument in Proposition~\ref{fact:rp2} is that in Binary BP, there is a one-to-one correspondence between simulation queries and thresholds in $(0, 1)$. %\textcolor{red}{[NSI: where does this $1/2$ come up below?]}

\begin{proposition}\label{prop:threshold}
    Given a simulation query $q = (\sigma, m)$ in Binary BP, the response $a_{q}$ is equal to $1$ if and only if the belief $p=Pr[\omega=1|s]$ of the receiver conditional on the private signal $s$ satisfies $p \geq \theta_q$, where
    %
    \begin{equation*}
        \theta_q = \frac{\sigma(m | \omega =1)}{\sigma(m | \omega = 1) + \sigma(m | \omega = 0)}.
    \end{equation*}
    %where the right-hand-side is a threshold 
    %\textcolor{red}{[NSI: should we name the threshold? and i don't see why it's less than 1/2.]}
\end{proposition}

This result implies that in Binary BP, there always exists a simulation query $q$ that can distinguish between any two receiver beliefs $p_{i}$, $ p_{j}$ such that $p_{i} \neq p_{j}$. Furthermore, any simulation query implies a partition on beliefs defined by a threshold.\footnote{Interestingly, this is not true in general; as we discuss in Section~\ref{}, simulation queries in non-binary settings may distinguish between three or more beliefs.}  We will use this in Section~\ref{sec:equilcomp} to argue that the optimal query policy of the sender can be characterized as choosing a set of thresholds.



==> paper/main_body/setting.tex <==
\section{Model and Preliminaries}\label{sec:setting}
%
%We first overview the Bayesian Persuasion setting in~\Cref{sec:bp}, before introducing the receiver-informed oracle in~\Cref{sec:model}.  
%
\xhdr{Bayesian Persuasion.}
%
We denote the set of possible world states by $\Omega$ and the set of receiver actions by $\cA$, where $d := |\Omega| < \infty$ and $A := |\cA| < \infty$. 
%
In the classic persuasion setting, it is assumed that state $\omega$ is drawn from some distribution $\vp$ over $\Omega$ which is known to both the sender and receiver. 
%
Sender and receiver utilities are given by utility functions $u_S : \Omega \times \cA \rightarrow \mathbb{R}$ and $u_R : \Omega \times \cA \rightarrow \mathbb{R}$ respectively. 
%
Both $u_S$ and $u_R$ are known to the sender. The sender commits to a messaging policy which maps states to messages.
%
\begin{definition}[Messaging Policy]\label{def:messaging}
    The sender's \emph{messaging policy} $\sigma : \Omega \rightarrow \cM$ is a (randomized) mapping from states to \emph{messages} in some message class $\cM$ such that $M := |\cM| < \infty$.  We will sometimes write $\sigma(m|\omega)$ to denote $\Pr[\sigma(\omega)=m]$.
\end{definition}
%
We use $\cM \ni m \sim \sigma(\omega)$ to denote a message sampled from $\sigma$ when the state is $\omega \in \Omega$.
%
The timing of the game is as follows: 1) the sender commits to a messaging policy $\sigma$; 2) the state $\omega$ is revealed to the sender; 3) the message $m \sim \sigma(\omega)$ is sent to the receiver; 4) the receiver chooses an action $a\in\cA$.\looseness-1

%
When the sender and receiver share a common prior $\vp$ it is without loss of generality to message according to the set of possible actions (i.e. $\cM = \cA$) via a revelation principle-style argument. (See~\cite{kamenica2011bayesian} for more details.)
%
Under this setting, a message has the interpretation of being the action that the sender is recommending the receiver to take. 
%
We say that the sender's messaging policy is \emph{Bayesian incentive-compatible} (BIC) if it is always in the receiver's best interest to follow the sender's action recommendations.\looseness-1 
%
\begin{definition}[Bayesian Incentive-Compatibility]\label{def:BIC}
    A messaging policy $\sigma : \Omega \rightarrow \cA$ is Bayesian incentive-compatible if for every action $a \in \cA$,
    %
    \begin{equation*}
        \mathbb{E}_{\omega \sim \vp}[u_R(\omega, m) | m] \geq \mathbb{E}_{\omega \sim \vp}[u_R(\omega, a) | m].
    \end{equation*}
    %
    %$\mathbb{E}_{\omega \sim \vp}[u_R(\omega, m) | m] \geq \mathbb{E}_{\omega \sim \vp}[u_R(\omega, a) | m]$. 
    %
    We assume that if the receiver is indifferent between two actions, she breaks ties in favor of the sender's recommended action.\looseness-1 
    %
\end{definition}  
%
\noindent The sender's optimal messaging policy $\sigma$ is given by the solution to the following linear program:
%
\begin{equation*}
\begin{aligned}
    \max_{\sigma} \; &\mathbb{E}_{\omega \sim \vp, m \sim \sigma(\omega)}[u_S(\omega, m)]\\
    %
    \text{ s.t. } \;\; \mathbb{E}_{\omega \sim \vp}[u_R(\omega, m) | m, \sigma] &\geq \mathbb{E}_{\omega \sim \vp}[u_R(\omega, a) | m, \sigma], \;\; \forall a \in \cA, m \in \cM
\end{aligned}
\end{equation*}
%
\iffalse
\begin{figure}[tbp]
    \centering
    \noindent \fbox{\parbox{0.95\textwidth}{
    \vspace{0.1cm}
    \textbf{Protocol: Bayesian Persuasion}
    
    \vspace{-0.2cm}
    %\noindent\rule{15.9cm}{0.4pt}
    \noindent\rule{15.1cm}{0.4pt}
    %\noindent\rule{13.2cm}{0.4pt}\vspace{1mm}
    \begin{enumerate}
        %\setcounter{enumi}{-1}
        \item Sender \emph{commits} to messaging policy $\sigma : \Omega \rightarrow \cM$.
        %
        \item Sender observes state $\omega \sim \vp_{\tau}$, where $\tau \sim \cP$.
        %
        \item Sender sends message $m \sim \sigma(\omega)$, receiver forms posterior $\vp_{\tau} | m$.
        %
        \item Receiver takes action $\arg\max_{a \in \cA} \mathbb{E}_{\omega \sim \vp_{\tau}}[u_R(\omega, a) | m]$.
    \end{enumerate}
    }}
    \caption{Description of the classic Bayesian Persuasion game between a sender and receiver.}
    \label{fig:bp}
\end{figure}
\fi 
%
%See~\Cref{fig:bp} for a succinct summary of the Bayesian Persuasion setting. 
%
The time it takes to compute the optimal messaging policy is $\mathcal{O}(\lp(dA, A^2 + dA))$, where $\lp(x,y)$ is the time it takes to solve a linear program with $x$ variables and $y$ constraints. 
%
Some of our results are specialized to the following \emph{binary} setting, which is itself a popular model of persuasion (see, e.g. \cite{parakhonyak2022persuasion, kosterina2022persuasion, hu2021robust, kolotilin2017persuasion} for various versions of this setting studied in the literature).\looseness-1
%
\begin{definition}[Binary Bayesian Persuasion]\label{def:bin}
    In the Binary Bayesian Persuasion setting, $\omega \in \{0, 1\}$, $a \in \{0, 1\}$, and the prior over states can be described by a single number $p := \mathbb{P}(\omega = 1)$. 
    %
    Furthermore, we assume the following utility functions for the sender and receiver: 
    \begin{equation*}
    \begin{aligned}
        u_S(\omega, a) = \mathbbm{1}\{\omega = 1\}, \;\;\;
        %
        u_R(\omega, a) = \mathbbm{1}\{\omega = a\}
    \end{aligned}
    \end{equation*}
    %$u_S(\omega, a) = \mathbbm{1}\{\omega = 1\}$, $u_R(\omega, a) = \mathbbm{1}\{\omega = a\}$. 
    %
    In other words, the sender always wants to incentivize the receiver to take action $a=1$, but the receiver only wants to take action $a=1$ whenever $\omega = 1$.
\end{definition}


==> paper/main_body/simulation_helps.tex <==
\subsection{The Geometry of Simulation Queries}\label{sec:helps}

\textcolor{red}{[NSI: STOPPED HERE]}

An immediate corollary of~\Cref{fact:rp2} is that in Binary BP, there is a one-to-one correspondence between simulation queries and thresholds in $(0, \frac{1}{2})$. 

\begin{corollary}\label{cor:threshold}
    Given a simulation query $q = (\sigma_q, m_q)$ in Binary BP, $a_{q, \tau^*} = m_q$ if and only if 
    %
    \begin{equation*}
        p_{\tau^*}[m_q] \geq \frac{\sigma_q(m_q | \omega \neq m_q)}{\sigma_q(m_q | \omega = m_q) + \sigma_q(m_q | \omega \neq m_q)},
    \end{equation*}
    %
    %$p_{\tau^*}[m_q] \geq \frac{\sigma_q(m_q | \omega \neq m_q)}{\sigma_q(m_q | \omega = m_q) + \sigma_q(m_q | \omega \neq m_q)}$, 
    %
     where $p_{\tau^*}[m]$ denotes the prior probability that receiver type $\tau^*$ places on the state $\omega$ equaling the recommended action $m$ (i.e. $p_{\tau^*}[m] = p_{\tau^*}$ if $m=1$ and $p_{\tau^*}[m] = 1 - p_{\tau^*}$ if $m=0$). 
\end{corollary}
%
\Cref{cor:threshold} implies that in Binary BP, there always exists a simulation query $q$ which can distinguish between any two receiver beliefs $p_{\tau}$, $ p_{\tau'}$ such that $p_{\tau} \neq p_{\tau'}$. Furthermore, any simulation query implies a partition on beliefs defined by a threshold.\footnote{Interestingly, this is not true in general; as we discuss in Section~\ref{}, simulation queries }  We will use this in Section~\ref{} to argue that the optimal query policy of the sender can be characterized as choosing a set of thresholds.
%
Similar intuition carries over to the general setting, although it may be possible to distinguish between three or more beliefs using a \emph{single} simulation query (unlike in Binary BP). 
%
The following is an example of a setting in which it is possible to distinguish between up to $d$ different beliefs using a single simulation query.\looseness-1 
%
\iffalse
\begin{example}\label{ex:sep-many}
    Suppose that there are $d$ states and $d$ actions, where $u_R(\omega, a) = \mathbbm{1}\{\omega = a\}$. 
    %
    Consider $d$ receiver beliefs $\vp_1, \ldots, \vp_d$ and let $\vp_i[\omega_i] = \frac{2}{d+1}$, $\forall i \in [d]$ and $\vp_i[\omega_j] = \frac{1}{d+1}$ for $j \neq i$.
    %
    Under this setting, receiver type $i$ will take action $a_i$ when $m = a_1$ if for all $j \neq 1$,
    %
    \iffalse
    \begin{equation*}
        \sigma(m = a_1| \omega_1) \cdot \frac{2}{d+1} \geq \sigma(m = a_1| \omega_j) \cdot \frac{1}{d+1}.
    \end{equation*}
    \fi 
    %
    %Therefore, $\vp_1$ will take action $a_1$ when $m = a_i$ if for all $j \neq 1$, 
    $\sigma(a_1| \omega_j) = 2 \sigma(a_1|\omega_1)$.\looseness-1 
    %
    %Now let us consider another receiver type $i \neq 1$. 
    %
    %Type $i$ will default to taking action $i$ under this messaging policy whenever $m=a_1$, since 
    %
    \iffalse
    \begin{equation*}
    \begin{aligned}
        \sigma(m | \omega_1) \cdot \frac{1}{d+1} &< 2\sigma(m|\omega_1) \cdot \frac{2}{d+1}\\
        %
        \sigma(m | \omega_1) \cdot \frac{1}{d+1} &< 2\sigma(m|\omega_1) \cdot \frac{1}{d+1}
    \end{aligned}
    \end{equation*}
    \fi 
    %where the first line is proportional to how much the receiver loses in expectation by not taking action $i \neq 1$ when recommended action $1$, and the second line is proportional to how much she loses in expectation by not taking action $j \neq i \neq 1$ when recommended action $1$.
\end{example}
\fi 
%
\begin{example}\label{ex:sep-many}
    Suppose that there are $d$ states and $d$ actions, where $u_R(\omega, a) = \mathbbm{1}\{\omega = a\}$. 
    %
    Consider $d$ receiver beliefs $\vp_1, \ldots, \vp_d$ and let $\vp_i[\omega_i] = \frac{2}{d+1}$, $\forall i \in [d]$ and $\vp_i[\omega_j] = \frac{1}{d+1}$ for $j \neq i$.
    %
    Under this setting, receiver type $i$ will take action $a_i$ when $m = a_1$ if for all $j \neq 1$,
    %
    \begin{equation*}
        \sigma(a_1| \omega_1) \cdot \frac{2}{d+1} \geq \sigma(a_1| \omega_j) \cdot \frac{1}{d+1}.
    \end{equation*}
    %
    Therefore, $\vp_1$ will take action $a_1$ when $m = a_i$ if for all $j \neq 1$, 
    $\sigma(a_1| \omega_j) = 2 \sigma(a_1|\omega_1)$. 
    %
    Now let us consider another receiver type $i \neq 1$. 
    %
    Type $i$ will default to taking action $i$ under this messaging policy whenever $m=a_1$, since 
    %
    \begin{equation*}
    \begin{aligned}
        \sigma(m | \omega_1) \cdot \frac{1}{d+1} &< 2\sigma(m|\omega_1) \cdot \frac{2}{d+1}\\
        %
        \sigma(m | \omega_1) \cdot \frac{1}{d+1} &< 2\sigma(m|\omega_1) \cdot \frac{1}{d+1}
    \end{aligned}
    \end{equation*}
    where the first line is proportional to how much the receiver loses in expectation by not taking action $i \neq 1$ when recommended action $1$, and the second line is proportional to how much she loses in expectation by not taking action $j \neq i \neq 1$ when recommended action $1$.
\end{example}
%
Since there are a finite number of receiver types, it suffices to consider a finite set of possible simulation queries without loss of generality. 
%
In the sequel, our goal is to determine the optimal adaptive/non-adaptive querying policy, given a set of valid queries as input. 
%
%However in~\Cref{sec:all-sep}, we describe a (computationally-inefficient) procedure for identifying this finite set of simulation queries. 
%
%While in~\Cref{sec:all-sep} we describe a (computationally-inefficient) procedure for identifying such a set of simulation queries, our goal is to determine the optimal querying policy \emph{given a set of unique queries}. 
%
%As such, we assume that the set of valid queries $\cQ$ is given as input to the problem instance. 

==> paper/main_body/unknown_type.tex <==
\section{How Should We Think About Querying?}\label{sec:think}
%
We begin with structural results which showcase intuition and will be useful later. 
%
We derive the sender's optimal messaging policy when there is uncertainty about the receiver's belief. 
%
Then we discuss geometric properties of simulation queries, illustrating how they benefit the sender.\looseness-1

%We begin by overviewing several structural results which will be useful in later results.
%%
%In~\Cref{sec:unknown_prior}, we derive the sender's optimal messaging policy whenever she has uncertainty about the receiver's beliefs.
%%
%In~\Cref{sec:helps}, we derive geometric properties of simulation queries, which will be useful for obtaining algorithms for querying.
%
\subsection{Optimal Persuasion Under Uncertainty}\label{sec:unknown_prior}
%
How should the sender send messages whenever she is uncertain about the receiver's belief?
%
Recall that when the receiver's prior is known, the sender can send messages according to the set of receiver actions (i.e. $\cM = \cA$).
%
%The same cannot be said in our setting, so we need to derive an analogous ``revelation principle'' 
When the sender has uncertainty about the receiver,
%
%It turns out that it suffices to consider 
$A^T$ messages suffice in the general setting and $T+1$ messages suffice in Binary BP.\looseness-1
%
\begin{restatable}{proposition}{rp}[Revelation Principle for Unknown Receiver Beliefs]\label{fact:rp2}
    It always suffices for the sender to use a message space of size $M = A^T$.
    %
    In Binary BP, it suffices to use $M = T + 1$ messages.\looseness-1
\end{restatable}
%
We can now characterize the sender's optimal messaging policy whenever she has uncertainty about the receiver's belief, both in the general setting (\Cref{thm:opt-sp}) and in Binary BP (\Cref{cor:opt-binary}).
%
The optimal messaging policy in the general setting follows readily from the above revelation principle for unknown receiver beliefs.
%
\begin{corollary}[Optimal Messaging Policy]\label{thm:opt-sp}
    For second-order prior $\cP$, the sender's optimal messaging policy $\sigma^*_{\cP}$ is given by the solution to the following linear program:\looseness-1
    %
    \begin{equation*}
    \begin{aligned}
        \sigma^*_{\cP} := \arg\max_\sigma \; &\mathbb{E}_{\tau \sim \cP}[\mathbb{E}_{\omega \sim \vp_{\tau}} [\mathbb{E}_{m \sim \sigma(\omega)}[u_S(\omega, m[\tau])]]]\\
        %
        \text{s.t. } \mathbb{E}_{\omega \sim \vp_{\tau}}[u_R(\omega, m[\tau]) | m, \sigma] &\geq \mathbb{E}_{\omega \sim \vp_{\tau}}[u_R(\omega, a) | m, \sigma], \forall a \in \cA, \tau \in \cT', m \in \cM
    \end{aligned}
    \end{equation*}
    %
    Here $m[\tau]$ denotes the $\tau$-th component of the message vector $m \in \cA^{T'}$, where $T' := |\cT'|$.
    %
    The time it takes to compute the solution to this linear program is $\mathcal{O}(\lp(d A^{T'}, T'A^{T'+1} + d A^{T'}))$.%, where $\lp(x,y)$ is the time it takes to solve a linear program with $x$ variables and $y$ constraints.
\end{corollary}
%
The form of the sender's optimal messaging policy may be further simplified in Binary BP.
%
In particular, the optimal messaging policy in Binary BP has the following interpretation: when receiving message $m_{i'}$, all receivers with belief $p$ such that $p \leq p_{i'}$ should take action $a=1$.
%
In order to simplify the exposition, we assume that $p_{\tau} \leq \frac{1}{2}$ for every receiver type $\tau \in \cT$.\footnote{This assumption is without loss of generality, since the sender can treat all receiver types with prior $\mathbb{P}(\omega = 1) \geq \frac{1}{2}$ as the same type without any loss in utility.}
%
\begin{restatable}{corollary}{optsp}[Optimal Messaging Policy; Binary BP]\label{cor:opt-binary}
In Binary BP, for a given set of receivers $\cT' := \{\tau_{L}, \tau_{L+1}, \ldots, \tau_{H-1}, \tau_{H}\}$ where $p_{L} >  p_{L-1} > \ldots > p_{H-1} > p_{H}$, the sender's optimal messaging policy can be computed in time $\mathcal{O}((T')^2)$. 
%
The optimal policy is given by $\sigma(m_{i^*}|1) = 1$, $\sigma(m_{i^*}|0) = \frac{p_{i^*}}{1-p_{i^*}}$, and $\sigma(0|0) = 1 - \frac{p_{i^*}}{1-p_{i^*}}$, %where $i^* := \arg\max_{i' \in [L,H]} \; \sum_{i=L}^{i'} \cP(\tau_i) \cdot \left(p_i + (1 - p_i) \cdot \frac{p_{i'}}{1-p_{i'}} \right)$.
%
% \begin{equation*}
% \begin{cases}
%     & \sigma(m_{i^*}|1) = 1\\
%     %
%     & \sigma(m_{i^*}|0) = \frac{p_{i^*}}{1-p_{i^*}}\\
%     %
%     & \sigma(0|0) = 1 - \frac{p_{i^*}}{1-p_{i^*}},
% \end{cases}
% \end{equation*}
%
where 
%
\begin{equation*}
    i^* := \arg\max_{i' \in [L,H]} \; \sum_{i=L}^{i'} \cP(\tau_i) \cdot \left(p_i + (1 - p_i) \cdot \frac{p_{i'}}{1-p_{i'}} \right).
\end{equation*}

%and sets $\sigma(m=m_{i^*} | \omega = 1) = 1$, $\sigma(m=m_{i^*} | \omega = 0) = \frac{p_{i^*}}{1-p_{i^*}}$, and $\sigma(m=0 | \omega = 0) = 1 - \frac{p_{i^*}}{1-p_{i^*}}$, where $i^* := \arg\max_{i' \in [L,H]} \; \sum_{i=L}^{i'} \mathbb{P}_{\cP(\cT')}(\tau_i) \cdot \left(p_i + (1 - p_i) \cdot \frac{p_{i'}}{1-p_{i'}} \right)$.
%
\end{restatable}
% 
